Convolutional Filtering with RKHS Algebras

In this paper, we develop a generalized theory of convolutional signal processing and neural networks for Reproducing Kernel Hilbert Spaces (RKHS). Leveraging the theory of algebraic signal processing (ASP), we show that any RKHS allows the formal definition of multiple algebraic convolutional models. We show that any RKHS induces algebras whose elements determine convolutional operators acting on RKHS elements. This approach allows us to achieve scalable filtering and learning as a byproduct of the convolutional model, and simultaneously take advantage of the well-known benefits of processing information in an RKHS. To emphasize the generality and usefulness of our approach, we show how algebraic RKHS can be used to define convolutional signal models on groups, graphons, and traditional Euclidean signal spaces. Furthermore, using algebraic RKHS models, we build convolutional networks, formally defining the notion of pointwise nonlinearities and deriving explicit expressions for the training. Such derivations are obtained in terms of the algebraic representation of the RKHS. We present a set of numerical experiments on real data in which wireless coverage is predicted from measurements captured by unmaned aerial vehicles. This particular real-life scenario emphasizes the benefits of the convolutional RKHS models in neural networks compared to fully connected and standard convolutional operators.

==> figures/algnn_one_layer.tex <==
%!TEX root = ../../lecture_\ell2_compile_handout/lecture_\ell2_handout.tex

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}

\def \myfactor {0.8}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks
\tikzstyle{filter} = [block,
                      minimum width  = 3.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=my_cp_col5]

% Control the color and size of nonlinearity blocks
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 2.5*\unit,
                             fill = my_cp_col4]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.7)}
\def \deltaoutput    {( 0.0,-1.2)}
\def \deltalayer     {3.2}
\def \deltaconnector {1.45}
\def \deltasigma     {( 3.8, 0.0)}
\def \deltasigmab    {( 3.5, 0.0)}

% The text that is displayed inside of filter blocks
\def \one {$\textcolor{white}{\displaystyle{\boldsymbol{y}^{\ell}_m = \sum_{n=1}^{N_{\ell-1}}h_{n,m}^{\ell} \ast\boldsymbol{x}_n^{\ell-1}}}$}

% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\textcolor{white}{\displaystyle{\boldsymbol{x}_{\ell} = {\eta_{\ell}} \Big[\, \boldsymbol{y}_{\ell} \, \Big]}}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{8}{8}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\boldsymbol{x}_{\ell\text{-}1}=\left(x_1^{\ell\text{-}1}, \hdots, x_{N_{\ell\text{-}1}}^{\ell\text{-}1}\right)$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input.east)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\boldsymbol{y}_\ell$} (L1 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.east) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- (aux1.north) node [right] {$\boldsymbol{x}_\ell=\left(x_1^{\ell}, \hdots, x_{N_{\ell}}^{\ell}\right)$} ;

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg}
      % Shading for Layer 1
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.5)
           node [filter, anchor = south west,
                 fill = black!5,
minimum width  = 7.5*\unit,
minimum height = 2.0*\unit,
]
        (layer)
        {};
       \path (layer.south west) ++ (0.0,0.0) node [above right] {Layer $\ell$};
   \end{pgfonlayer}

\end{tikzpicture}}


==> figures/asp_diagrams/fig2_tikz_source.tex <==
%!TEX root = ../../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%



%-- Viridis Color Palette
%% ----- Viridis color palette -----
\definecolor{my_cp_col1}{RGB}{253, 231, 37}
\definecolor{my_cp_col2}{RGB}{180, 222,44}
\definecolor{my_cp_col3}{RGB}{94, 201, 98}
\definecolor{my_cp_col4}{RGB}{33, 145, 140}
\definecolor{my_cp_col5}{RGB}{59, 82, 139}
\definecolor{my_cp_col6}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {4}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                                      
\tikzstyle{vectorspace} = [set, 
                             fill=my_cp_col5,
                             minimum width  = 2.5*\unit,
                             minimum height = 1.5451*\unit]
                             
\tikzstyle{endomorphisms} = [vectorspace,
                              fill=my_cp_col4]
                                
\tikzstyle{algebra} = [endomorphisms,
                        fill=my_cp_col2,
                         minimum width  = 2.5*\unit,
                        minimum height = 1.5451*\unit]

\tikzstyle{rec_box} = [endomorphisms,
                         rounded corners = 0*\unit,
                        fill=my_cp_col2,
                         minimum width  = 2.5*\unit,
                        minimum height = 1.5451*\unit]



\tikzstyle{dot} = [circle,
                    minimum width  = 0.12*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace, fill opacity=1] (M0) {};
   \path (M0.south) ++ (0, 0.2) node [above, color=my_cp_col2] {$\mathcal{H}$};
   
   % Element of the vector space
   \path (M0) ++ (-1,0.2) node [dot,color=my_cp_col2] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=my_cp_col2] {$\boldsymbol{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (1,0.2) node [dot,color=my_cp_col2] (ex) {};
   \path (ex.south) node [below, color=my_cp_col2] {$\rho(\boldsymbol{a})\boldsymbol{x}$};      
              

% Comment about where the signals living in H
 \path (M0.south) ++ (0,0) node [] (Htext) {};
 \path (Htext.south) node [below, color=my_cp_col6,align=center] {Vector Space
   (Signals)}; 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 1) 
         node [endomorphisms, anchor=south, fill opacity=1] (End0) {};
   \path (End0.north) ++ (0.0, -0.2) node [below, color=my_cp_col6] {$\mathcal{B}\left(\mathcal{H}\right)$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.6) node [dot,color=my_cp_col6] (e) {};      
   %\path (e) node [right] {$\rho(\boldsymbol{a})$};    
   \path (e.center) ++ (0.5,0.25) node [color=my_cp_col6] {$\rho(\boldsymbol{a})$}; 
   
   % Arrow going from x to Ex
   \path (e)+(-1,0.77) coordinate (c1);
   \path (e)+(1,0.77) coordinate (c2);   
   \path [draw, -stealth, line width=0.8,color=my_cp_col3] (x) .. controls (c1) and (c2) .. (ex);   

  

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Algebra %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east, fill opacity=1] (A) {};   
   \path (A.north) ++ (0,-0.2) node [below,color=my_cp_col6] {$\mathcal{A}$};
   \path (A.center) ++ (-0.25,0) node [below,color=my_cp_col6] {$\boldsymbol{a}$};  
   %\path (A.south) ++ (0,0.75) node [below,color=black, align=center] {};  
    
%  \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.6) node [dot,color=my_cp_col6] (a1) {}; 
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.1) coordinate (c1);
   \path (End0.north) + (-1,-0.1) coordinate (c2);   
   \path [draw, -stealth,line width = 1,color=my_cp_col5,  opacity=1] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=black,opacity=1] {$\rho$};
   
   
% Comment about where the signals living in H
 \path (A.south) ++ (0,0) node [] (Atext) {};
 \path (Atext.south) node [below, color=my_cp_col6,align=center] {Algebra
   (Filters)}; 


   
   




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  C O M M E N T S   A N D   T E X T   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
   
\path (A.south) ++ (0, -1) node [rec_box, anchor=north, fill opacity=0.2,color=my_cp_col1] (rectext) {};
   
% Comment about where the signals living in H
 \path (A.south) ++ (0,-0.9) node [] (Atext) {};
 \path (Atext.south) node [below, color=my_cp_col3,align=center] { $\ccalA\Rightarrow$ \textbf{Fundamental Laws}  \\
   \textbf{of convolution}};            
          
 % Comment about where the signals living in H
 \path (A.south) ++ (0,-1.8) node [] (Htext) {};
 \path (Htext.south) node [below, color=my_cp_col5] {$\ccalH\Rightarrow$ \textbf{Information (data)} };       
 
 
  % Comment about where the signals living in H
 \path (A.south) ++ (0,-2.4) node [] (Endtext) {};
 \path (Endtext.south) node [below, color=my_cp_col4] {$\rho\Rightarrow$ \textbf{Implements filters}};    

\end{tikzpicture}
}







==> figures/gnn_block_diagram_single_feature_uncolored_01.tex <==
% !TEX root = ../compiler_paper.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% COLORS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%--- Viridis Color Palette
\definecolor{my_cp_col1}{RGB}{253, 231, 37}
\definecolor{my_cp_col2}{RGB}{94, 201, 98}
\definecolor{my_cp_col3}{RGB}{33, 145, 140}
\definecolor{my_cp_col4}{RGB}{59, 82, 139}
\definecolor{my_cp_col5}{RGB}{68, 1, 84}

%--- Secondary Viridis Color Palette 
\definecolor{my_cp2_col1}{RGB}{255,255,217}
\definecolor{my_cp2_col2}{RGB}{237,248,177}
\definecolor{my_cp2_col3}{RGB}{199,233,180}
\definecolor{my_cp2_col4}{RGB}{127,205,187}
\definecolor{my_cp2_col5}{RGB}{65,182,196}
\definecolor{my_cp2_col6}{RGB}{29,145,192}
\definecolor{my_cp2_col7}{RGB}{34,94,168}
\definecolor{my_cp2_col8}{RGB}{37,52,148}
\definecolor{my_cp2_col9}{RGB}{8,29,88}







%%------------- Scaling Factor ---------

\def \myfactor {0.65}
\def \unit  {\myfactor cm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% Definition of Blocks %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = gray,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 5*\unit,
                      minimum height = 1.7*\unit,
                      fill = my_cp2_col7,
                      fill opacity=1,
                      text opacity=1]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 5*\unit,
                             fill = my_cp2_col3,
                             fill opacity=1,
                             text opacity=1]

% Control the color and size of Pooling blocks 
\tikzstyle{pooling} = [ filter,
                             minimum width  = 3*\unit,
                             fill = my_cp5_col2]

% Control separation between blocks
\def \deltainput     {( 0.0,-2.7*\unit)}
\def \deltaoutput    {( 0.0,-1.2)}
\def \deltalayer     {4}
\def \deltaconnector {1.45}
\def \deltasigma     {( 12.65*\unit, 0.0)}



%%-----------------------------------------------------------
%%---- The text that is displayed inside of filter blocks
%%-----------------------------------------------------------

\def\one{$\textcolor{my_cp2_col2}{\displaystyle{g_{1}  = \sum_{v\in\ccalV_{1}}w_{1,v}k_{v} \ast f}}$}

\def\two{$\textcolor{my_cp2_col2}{\displaystyle{g_2  =\sum_{v\in\ccalV_{2}}w_{2,v}k_{v}\ast h_{1}}}$}

\def \three {$\textcolor{my_cp2_col2}{\displaystyle{g_3  = \sum_{v\in\ccalV_{3}}w_{3,v}k_{v}\ast h_{2}}}$}




%%--------------------------------------------------------------
%%---- The text that is displayed inside of nonlinearity blocks
%%--------------------------------------------------------------

\def \sigmaone   {$\textcolor{black}{\displaystyle{h_{1} = {\eta} \Big[\, g_{1} \, \Big]}}$}
\def \sigmatwo   {$\textcolor{black}{\displaystyle{h_{2}= {\eta} \Big[\, g_{2} \, \Big]}}$}
\def \sigmathree {$\textcolor{black}{\displaystyle{h_{3} = {\eta} \Big[\, g_3 \, \Big]}}$}
% \def \proyone   {$\displaystyle{\boldsymbol{x}_{1} = {P_{1}} \Big[\, \boldsymbol{z}_1 \, \Big]}$}
% \def \proytwo   {$\displaystyle{\boldsymbol{x}_{2} = {P_{2}} \Big[\, \boldsymbol{z}_2 \, \Big]}$}
% \def \proythree   {$\displaystyle{\boldsymbol{x}_{3} = {P_{3}} \Big[\, \boldsymbol{z}_3 \, \Big]}$}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\fontsize{9}{9}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$f$};
  
  
  %%--------------------------------------
  %%------------  Layer 1  -------------------
  %%--------------------------------------
  
  % Draw Layer 1 Filter block and Feature block
  \path (input.east)   ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$g_1$} (L1 F1.west);



  %%--------------------------------------
  %%------------  Layer 2  -------------------
  %%--------------------------------------
  
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$g_2$} (L2 F1.west);

  
  
  
   %%--------------------------------------
   %%------------  Layer 3  -------------------
   %%--------------------------------------
   
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$g_3$} (L3 F1.west);




  %%--------------------------------------
  %%----- Connections across layers -----------
  %%--------------------------------------
  
  % From input to layer 1
  \path[draw, -stealth] (input.east) -- (L1 Filter1.north);
  
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- node [below right] {$h_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$h_1$} (L2 Filter1.north);
                                      
  % From layer 2 to layer 3
  \path (L2 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F1.south) -- node [below right] {$h_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$h_2$} (L3 Filter1.north);
                                      
  % From layer 3 to output
  \path[draw, -stealth] (L3 F1.south) -- ++ \deltaoutput -- ++ (0.5, 0) 
                        node [right]{$f_{\text{out}}$};



  %%------------------------------------------
  %%----- Light shades to signify layer groups --------
  %%------------------------------------------
  
  \begin{pgfonlayer}{bg} 
      %
      % Shading for Layer 1
      %  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 1};
      %
      % Shading for Layer 2  
      %
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 2};
      %
      % Shading for Layer 3  
      %
      \path (L1 Filter1.west |- L3 F1.south)  ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 3};  
    \end{pgfonlayer}

\end{tikzpicture}} 


==> figures/gnn_block_diagram_single_feature_uncolored_01__alejandro_parada_s_conflicted_copy_2024-06-24_.tex <==
% !TEX root = ../compiler_paper.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% COLORS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%--- Viridis Color Palette
\definecolor{my_cp_col1}{RGB}{253, 231, 37}
\definecolor{my_cp_col2}{RGB}{94, 201, 98}
\definecolor{my_cp_col3}{RGB}{33, 145, 140}
\definecolor{my_cp_col4}{RGB}{59, 82, 139}
\definecolor{my_cp_col5}{RGB}{68, 1, 84}

%--- Secondary Viridis Color Palette 
\definecolor{my_cp2_col1}{RGB}{255,255,217}
\definecolor{my_cp2_col2}{RGB}{237,248,177}
\definecolor{my_cp2_col3}{RGB}{199,233,180}
\definecolor{my_cp2_col4}{RGB}{127,205,187}
\definecolor{my_cp2_col5}{RGB}{65,182,196}
\definecolor{my_cp2_col6}{RGB}{29,145,192}
\definecolor{my_cp2_col7}{RGB}{34,94,168}
\definecolor{my_cp2_col8}{RGB}{37,52,148}
\definecolor{my_cp2_col9}{RGB}{8,29,88}







%%------------- Scaling Factor ---------

\def \myfactor {0.65}
\def \unit  {\myfactor cm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% Definition of Blocks %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = gray,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 5*\unit,
                      minimum height = 1.7*\unit,
                      fill = my_cp2_col7,
                      fill opacity=1,
                      text opacity=1]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 5*\unit,
                             fill = my_cp2_col3,
                             fill opacity=1,
                             text opacity=1]

% Control the color and size of Pooling blocks 
\tikzstyle{pooling} = [ filter,
                             minimum width  = 3*\unit,
                             fill = my_cp5_col2]

% Control separation between blocks
\def \deltainput     {( 0.0,-2.7*\unit)}
\def \deltaoutput    {( 0.0,-1.2)}
\def \deltalayer     {4}
\def \deltaconnector {1.45}
\def \deltasigma     {( 12.65*\unit, 0.0)}



%%-----------------------------------------------------------
%%---- The text that is displayed inside of filter blocks
%%-----------------------------------------------------------

\def\one{$\textcolor{my_cp2_col2}{\displaystyle{g_{1}  = \sum_{i\in\ccalI_{1}}w_{1,i}k_{i} \ast f}}$}

\def\two{$\textcolor{my_cp2_col2}{\displaystyle{g_2  =\sum_{i\in\ccalI_{2}}w_{2,i}k_{i}\ast h_{1}}}$}

\def \three {$\textcolor{my_cp2_col2}{\displaystyle{g_3  = \sum_{i\in\ccalI_{3}}w_{3,k}k_{i}\ast h_{2}}}$}




%%--------------------------------------------------------------
%%---- The text that is displayed inside of nonlinearity blocks
%%--------------------------------------------------------------

\def \sigmaone   {$\textcolor{black}{\displaystyle{h_{1} = {\eta_{1}} \Big[\, g_{1} \, \Big]}}$}
\def \sigmatwo   {$\textcolor{black}{\displaystyle{h_{2}= {\eta_{2}} \Big[\, g_{2} \, \Big]}}$}
\def \sigmathree {$\textcolor{black}{\displaystyle{h_{3} = {\eta_{3}} \Big[\, g_3 \, \Big]}}$}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\fontsize{9}{9}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$f$};
  
  
  %%--------------------------------------
  %%------------  Layer 1  -------------------
  %%--------------------------------------
  
  % Draw Layer 1 Filter block and Feature block
  \path (input.east)   ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$g_1$} (L1 F1.west);



  %%--------------------------------------
  %%------------  Layer 2  -------------------
  %%--------------------------------------
  
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$g_2$} (L2 F1.west);

  
  
  
   %%--------------------------------------
   %%------------  Layer 3  -------------------
   %%--------------------------------------
   
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$g_3$} (L3 F1.west);




  %%--------------------------------------
  %%----- Connections across layers -----------
  %%--------------------------------------
  
  % From input to layer 1
  \path[draw, -stealth] (input.east) -- (L1 Filter1.north);
  
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- node [below right] {$h_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$h_1$} (L2 Filter1.north);
                                      
  % From layer 2 to layer 3
  \path (L2 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F1.south) -- node [below right] {$h_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$h_2$} (L3 Filter1.north);
                                      
  % From layer 3 to output
  \path[draw, -stealth] (L3 F1.south) -- ++ \deltaoutput -- ++ (0.5, 0) 
                        node [right]{$h_{\text{out}}$};



  %%------------------------------------------
  %%----- Light shades to signify layer groups --------
  %%------------------------------------------
  
  \begin{pgfonlayer}{bg} 
      %
      % Shading for Layer 1
      %  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 1};
      %
      % Shading for Layer 2  
      %
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 2};
      %
      % Shading for Layer 3  
      %
      \path (L1 Filter1.west |- L3 F1.south)  ++ (-0.4,-0.7)
           node [filter, anchor = south west,
                 fill = black!5, 
                 minimum width  = 14*\unit,
                 minimum height = 2.8*\unit,] 
        (layer)
        {}; 
       \path (layer.south west) ++ (0.0,-0.1) node [above right] {Layer 3};  
    \end{pgfonlayer}

\end{tikzpicture}} 


==> figures/one_layer.tex <==
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron,  fill=black!50];
    \tikzstyle{realinput neuron}=[circle,draw,minimum size=17pt,inner sep=0pt, fill=white!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=12em, text centered]

%\foreach \name / \y in {2.5}
 %           \node[realinput neuron, pin=left:x] (I) at (-0.8*\layersep,-\y) {};

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron] (I-\name) at (0,-\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};



    
    
    %\foreach \source in {1,...,4}
    %    \foreach \dest in {1,...,5}
     %       \path (I) edge (I-\source);

    
    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1}
            \path (I-\source) edge (H-\dest);

   
    % Annotate the layers
   \node[annot,left of=H-1, node distance=-1cm ] {\begin{align*} h_{l,4,1}(t)&=H^{l,4,1}_{1} k(t^{l,4,1}_1,t)\\&+H^{l,4,1}_{2} k(t^{l,4,1}_{2},t)
 \end{align*}};

    
    \node[annot,right of=I-4, node distance=-2cm ] {\begin{align*}y_{l,4}(t)&=Y^{l,4}_1 k(t^{l,4}_1,t)\\&+Y^{l,4}_2 k(t^{l,4}_2,t)\end{align*}};

\node[annot,right of=I-1, node distance=-2cm ] {\begin{align*}y_{l,1}(t)&=Y^{l,1}_1 k(t^{l,1}_1,t)\\&+Y^{l,1}_2 k(t^{l,1}_2,t)\end{align*}};

    \node[annot,above of=H-1, node distance=1.1cm ] {\begin{align*} h_{l,1,1}(t)&=H^{l,1,1}_1 k(t^{l,1,1}_1,t)\\&+H^{l,1,1}_2 k(t^{l,1,1}_2,t)\end{align*}};
    
    
    \node[annot,right of=H-1, node distance=1cm ] {$ z_{l,1}(t)$};
    
\end{tikzpicture}

==> v35/sec_background_rkhs.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Basic Preliminaries}
\label{sec_appendix_basic_prelim}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Sub - Section %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Auxiliary Results}


Now, we turn our attention to results where we have a general description of how kernels can be built from certain types of functions and their intricate relationship with exponential maps. To do so, we start considering the following definitions.






%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 2.4~\cite{paulsen2016introduction})
\label{thm_K_from_basis_general}
Let $\ccalH(K)$ be an RKHS on $\ccalT$ with reproducing kernel $K$. If $\{ e_{s}: s\in\ccalS \}$ is an orthonormal basis for $\ccalH$, then
%
%
%
\begin{equation}\label{eq_K_sum_eigenvec}
K(u,v)
   =
    \sum_{i=1}^{\infty}
            \overline{e_{i}(u)}
            e_{i}(v)
            ,
\end{equation}
%
%
%
where this series converges pointwise.
\end{theorem}

%%-------- End of Theorem ----------------






As one can expect, specific attributes of $K(u,v)$ influence the norm associated with $\ccalH (K)$. In the case of kernels obtained from symbols and the box product, this can be formalized in the following theorem.



%%---------------------------------------------------
%%------------ T H E O R E M -----------------
%%--------------------------------------------------

\begin{theorem}[Theorem 11.3~\cite{paulsen2016introduction}]
\label{thm_kernel_from_box_prod}
%
Let $\ccalT$ be a set, let $(\ccalU, \mu)$ be a measure space, let $S(u,v): \ccalT \times \ccalU \to \mbC$ be square integrable in the $v$ variable and let $K: \ccalT\times \ccalT \to \mbC$ be the kernel function given by $K(u,z) = \left( S\square S^{\ast} \right)(u,z) $. Then $\left\lbrace  T_{S}\left\lbrace g \right\rbrace: g\in L^{2}(\ccalY,\mu)  \right\rbrace = \ccalH (K)$ and for $f\in\ccalH (K)$ we have that
%
%
%
\begin{equation}
 \left\Vert 
       f
 \right\Vert_{\ccalH (K)}
       =
       \inf 
           \left\lbrace 
                 \Vert g \Vert_{2}
                      :
                       f = T_{S} \{ g \}
           \right\rbrace
           .
\end{equation}
%
%
%
\end{theorem}

%%---------- End of Theorem ------------











%%-------------------------------------
%%---------- DEFINITION ---------------
%%-------------------------------------

\begin{definition}[~\cite{paulsen2016introduction}]\label{def_neg_def_func}
A function $\psi: \ccalX\times\ccalX \to \mbC$ is called conditionally negative definite if and only if, given $x_1, \ldots, x_n \in \ccalX$ and $\alpha_1, \ldots, \alpha_n \in \mbC$ such that $\sum_{j=1}^{n}\alpha_j = 0$, we have
%
%
%
\begin{equation}
\sum_{i,j=1}^{n}
       \overline{\alpha}_{i}\alpha_{j}
             \psi (x_i , x_j) 
             \leq 0
             .
\end{equation}
%
%
%
The function $\psi$ is called negative definite provided that this later inequality is met for all $\alpha_1, \ldots, \alpha_n \in \ccalX$.
\end{definition}

%%-------- End of Definition ----------




%%-------------------------------------
%%---------- DEFINITION ---------------
%%-------------------------------------

\begin{definition}[~\cite{paulsen2016introduction}]\label{def_neg_def_adjnt}
A conditionally negative definite function $\psi: \ccalX\times\ccalX \to \mbC$ is called self-adjoint provided that $\psi (y,x) = \overline{\psi (x,y)}$ and symettric provided that $\psi (y,x) = \psi (x,y)$.
\end{definition}

%%-------- End of Definition ----------


With Definitions~\ref{def_neg_def_func} and~\ref{def_neg_def_adjnt} at hand, we are ready to the so called Schoenberg's generator theorem, which leverages conditional negative definite functions and the exponential map to build families of kernels.


%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 9.7~\cite{paulsen2016introduction})
\label{thm_gen_kernel_exp}
The function $\psi: \ccalX \times \ccalX \to \mbC$ is a self-adjoint conditionally negative definite function if and only if the function $K_{t} = e^{-t\psi}$ is a kernel function for all $t>0$.
\end{theorem}

%%-------- End of Example ----------------


An interesting aspect of Theorem~\ref{thm_gen_kernel_exp} is that, it provides a concrete formula to generate kernels from negative definite functions exploiting the exponential map. This attribute endows the family of kernels $K_t$ with the structure of a semigroup and it formally allows one to capture time varying signals that are formally associated to an RKHS for each value of time. A similar result is derived in~\cite{paulsen2016introduction} considering the parametrization given by $L_t = t/(t+\psi(x,y))$ -- see Appendix~\ref{sec_appendix_basic_prelim}.







%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 9.9~\cite{paulsen2016introduction})
Let $\psi: \ccalX \times \ccalX \to \mbC$ with $\mathfrak{Re}\{ \psi(x,y) \}\geq 0$ for all $x,y\in\ccalX$. Then $\psi$ is self-adjoint and conditionally negative definite if and only if the function $L_t = t/(t+\psi(x,y))$ is a kernel function for all $t>0$.
\end{theorem}

%%-------- End of Example ----------------








%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Sub - Section %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS and Integral Operators}
\label{sub_sec_Ts_Tk_relationship}

Since the functions $\varphi_i$ constitute an orthonormal basis in $L_{2}(\ccalT,\mu)$, we can compute the inner product $\langle , \rangle_{\ccalH(K)}$ as follows
%
%
%
\begin{equation}
\left\langle 
   f
   ,
   g
\right\rangle_{\ccalH(K)}
=
\left\langle 
      \sum_{i}\langle 
                    f
                    ,
                    \varphi_i
              \rangle_{L_{2}}      
              \varphi_i
       ,
        \sum_{i}\langle 
                    g
                    ,
                    \varphi_i
              \rangle_{L_{2}}      
              \varphi_i
\right\rangle_{\ccalH(K)}
,
\end{equation}
%
%
%
then rearranging terms and exploiting the linearity properties of the inner products we have that
%
%
%
\begin{equation}
\left\langle 
   f
   ,
   g
\right\rangle_{\ccalH(K)}
=
\sum_{i=1}^{\infty}
   \left\Vert 
         \varphi_i
   \right\Vert_{\ccalH(K)}^{2}
         \langle
             f
             ,
             \varphi_i
         \rangle_{L_2} 
          \langle
             g
             ,
             \varphi_i
         \rangle_{L_2}   
         .
\end{equation}
%
%
%
To find the value of
%
%
$
 \left\Vert 
         \varphi_i
   \right\Vert_{\ccalH(K)}^{2}
$
%
%
we take into account that
%
%
%
\begin{equation}
\varphi_{i}(v)
=
\left\langle
   \varphi_{i}
   ,
   k_{v}
\right\rangle_{\ccalH(K)}
=
\left\langle
      \varphi_{i}
      ,
      \sum_{j=1}^{\infty}
          \sigma_{j}
          \varphi_{j}
          \varphi_{j}(v)
\right\rangle_{\ccalH(K)}
,
\end{equation}
%
%
%
which leads to
%
%
%
\begin{equation}\label{eq_norm_squared_in_HK_varphi}
\varphi_{i}(v)
     =
     \sigma_{i}
     \varphi_{i}(v)
     \left\Vert
          \varphi_{i}
     \right\Vert_{\ccalH(K)}^{2}
     \Rightarrow
     \left\Vert
          \varphi_{i}
     \right\Vert_{\ccalH(K)}^{2}
     =
     \frac{1}{\sigma_i}
     .
\end{equation}
%
%
%
We can see then that $e_i = \varphi_{i}\sqrt{\sigma_i}$ constitutes an orthonormal basis for $\ccalH(K)$.








%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%    S U B  - S E C T I O N    %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Fr\'echet Derivatives}



%%---------------------------------
%%-------- DEFINITION -------------
%%---------------------------------

\begin{definition}\label{def_frechet_derivative}

Let $\ccalH_1$ and $\ccalH_2$ two normed vector spaces and let $\ccalU\subset\ccalH_1$ be an open subset of $\ccalH_1$. We say that the function $F: \ccalH_1 \to \ccalH_2$ is Fr\'echet differentiable at $\boldsymbol{u}\in\ccalU$ if there exists a linear bounded operator $\bbD_{F}(\boldsymbol{u}):\ccalH_1 \to \ccalH_2$ such that
%
%
%
\begin{equation}\label{eq_def_frechet_derivative_1}
\lim_{\Vert \boldsymbol{d}\Vert\to 0}  
      \frac{\left\Vert
                  F(\boldsymbol{u}+\boldsymbol{d})
                  -
                  F(\boldsymbol{u})
                  +
                  \bbD_{F}(\boldsymbol{u})\{ \boldsymbol{d} \}
             \right\Vert}{\left\Vert 
                  \boldsymbol{d} 
             \right\Vert}
            =
            0
            ,
\end{equation}
%
%
%
which can be written as
%
%
%
\begin{equation}\label{eq_def_frechet_derivative_2}
F(\boldsymbol{u}+\boldsymbol{d}) = F(\boldsymbol{u}) + \bbD_{F}(\boldsymbol{u})\{ \boldsymbol{d} \} + o(\boldsymbol{d})    
.
\end{equation}
%
%
%
We refer to $\bbD_{F}(\boldsymbol{u})\{ \boldsymbol{d} \}$ as the Fr\'echet derivative of $F$ evaluated at $\boldsymbol{u}$ acting on $\boldsymbol{d}$.
\end{definition}

%%------- End of Definition -------



% If we want to think in a general way about the meaning of the Fr\'echet derivative, we should think about it as an operator acting on $d$ which can also be considered as the \textit{direction} of the derivative. To clarify this point, let us consider the following example.


% %%----------------------------------
% %%---------- EXAMPLE ---------------
% %%----------------------------------

% \begin{example}\normalfont 
% Let $F: M_{n\times n} \to M_{n\times n}$  be given by $F(\boldsymbol{x}) =  \boldsymbol{x}^2$. Then, to find the Fr\'echet derivative of $F$ we consider the difference between $F(\boldsymbol{x})$ and $F(\boldsymbol{x} + \boldsymbol{d})$, where $\boldsymbol{x}, \boldsymbol{d}\in M_{n\times n}$.
% %
% %
% %
% \begin{equation}\label{eq_ex_1}
% F(\boldsymbol{x} + \boldsymbol{d})
% -
% F(\boldsymbol{x}) 
% =
% \left( 
%       \boldsymbol{x} + \boldsymbol{d} 
% \right)^2
% -
% \boldsymbol{x}^2
% .
% \end{equation}
% %
% %
% %
% If we expand and cancel out common terms on the right hand side of the previous equation we have
% %
% %
% %
% \begin{equation}\label{eq_ex_2}
% F(\boldsymbol{x} + \boldsymbol{d})
% -
% F(\boldsymbol{x}) 
% =
% \boldsymbol{xd}
% +
% \boldsymbol{dx}
% .
% \end{equation}
% %
% %
% %
% If we compare~\eqref{eq_ex_2} with~\eqref{eq_def_frechet_derivative_2} we conclude that the Fr\'echet derivative of $F$ at $\boldsymbol{x}$, is the operator $\bbD_{F}(\boldsymbol{x}): M_{n\times n} \to M_{n\times n}$ whose action on $\boldsymbol{d}\in M_{n\times n}$ is given by
% %
% %
% %
% \begin{equation}
% \bbD_{F}(\boldsymbol{x})
%      \{ \boldsymbol{d} \}
%      =
%      \boldsymbol{xd}
%      +
%      \boldsymbol{dx}
%      ,
% \end{equation}
% %
% %
% %
% this is, the Fr\'echet derivative of $F$ at $\boldsymbol{x}$ is the operator
% %
% %
% %
% \begin{equation}
% \bbD_{F}(\boldsymbol{x})
%      \{ \cdot \}
%      =
%      \boldsymbol{x}(\cdot)
%      +
%      (\cdot)\boldsymbol{x}
%      . 
% \end{equation}
% %
% %
% %
% \end{example}

% %%-------- End of Example ----------

% It is important to remark that the role of the previous Example is to emphasize that for the calculation of a general Fr\'echet derivative one evaluates the difference between a function at a given point, $\boldsymbol{u}$, and its delay version $\boldsymbol{u}+\boldsymbol{d}$. Then, one finds the Fr\'echet derivative of $F$ at $\boldsymbol{u}$ focusing on those linear terms acting on $\boldsymbol{d}$.











==> v35/sec_derivatives_wrt_filter_coefficients.tex <==
%!TEX root =../compiler_paper.tex





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Derivatives w.r.t. Filter Coefficients}



% Consider the loss $\ell(r,y)=\frac{1}{2}\|r-y\|_H^2$.

% We can write
% \begin{align}
%     \ell(r,y)&=\frac{1}{2}\sum_{i=1}^{N_Y}\sum_{j=1}^{N_Y} Y_i Y_j k(t_i^Y,t_j^Y) - \sum_{i=1}^{N_Y}\sum_{j=1}^{N_R} Y_i R_n k(t_i^Y,t_j^R) +\text{const}\\
%     &=\frac{1}{2}\mathbf Y^H\mathbf K_{YY} \mathbf Y-\mathbf Y^H\mathbf K_{YR} \mathbf R
% \end{align} 

% where $\mathbf Y=(Y_1,Y_2,\ldots,Y_{N_Y})^H$ and $\mathbf R=(R_1,R_2,\ldots,R_{N_R})^H$ 
% In addition 

% \begin{align}
%     \mathbf Y= \text{RELU}(\mathbf Z^{ln})
% \end{align} 

% where $\mathbf Z^{ln}$ collects the coefficients of the unique (n=1)  signal $z^{ln}(t)$ formed in the previous layer $l=L-1$  as

% \begin{align}z^{ln}(t)=\sum_m  y^{lm}(t)*h^{lmn}(t)
% \end{align}

% which can be put in terms of the coefficients as

% \begin{align}\mathbf z^{ln}(t)&=\sum_m  y^{lm}(t)*h^{lmn}(t)
% \end{align}
% which corresponds to 

% \begin{align}\sum_{i=1} Z_i^{ln} k(t_i^{ln},t)=\sum_m\sum_j\sum_p  Y^{lm}_jH^{lmn}_p k(t_j^{lm}+t^{lmn}_p,t)
% \end{align}

% This implies that for each of  point $j$ in each  input $m$ and for each input $p$ in each  filter $m$ there is an index $i$ for a new kernel of $z^{ln}(t)$. This is given in the next identities and described by the ensuing figure

% \textcolor{blue}{
% \begin{align}
% t_i^{ln}&=t^{lm}_j+t^{lmn}_p\\
% Z_i^{ln}&=Y^{lm}_j H^{lmn}_p\label{eq:Zi}
% \end{align}
% }



% %%----------------------------
% %%---------- FIGURE ----------
% %%----------------------------

% \begin {figure}%[!hbtp]
% \centering
% %\begin{adjustbox}{width=\textwidth}
% \input{figures/one_layer.tex}
% %\end{adjustbox}
% \caption{Example to illustrate how the coefficients of the inputs and filters combine in one layer. All four inputs and filters are assumed to contain two kernels. The signal $z_{1n}(t)$ is the sum of the convolutions and collects all combinations of coefficients and it is composed of $4\times 2\times 2=16$ kernels. }
% \label{fig:onelayer}
% \end{figure}

% %%------ End of Figure -------




% The sum of convolutions for the example in Fig. \ref{fig:onelayer} is given by  
% \begin{align}
% z_{l1}(t)&=Y^{l,1}_1H^{l,1,1}_1 k(t^{l,1}_1+t^{l,1,1}_1)\\
% &+Y^{l,1}_1H^{l,1,1}_2 k(t^{l,1}_1+t^{l,1,1}_2)\\
% &+Y^{l,1}_2H^{l,1,1}_1 k(t^{l,1}_2+t^{l,1,1}_1)\\
% &+Y^{l,1}_2H^{l,1,1}_2 k(t^{l,1}_2+t^{l,1,1}_2)\\
% &+Y^{l,2}_1H^{l,2,1}_1 k(t^{l,2}_1+t^{l,2,1}_1)\\
% &+Y^{l,2}_1H^{l,2,1}_2 k(t^{l,2}_1+t^{l,2,1}_2)\\
% &+Y^{l,2}_2H^{l,2,1}_1 k(t^{l,2}_2+t^{l,2,1}_1)\\
% &+Y^{l,2}_1H^{l,2,1}_2 k(t^{l,2}_2+t^{l,2,1}_2)\\
% &+Y^{l,3}_1H^{l,3,1}_1 k(t^{l,3}_1+t^{l,3,1}_1)\\
% &+Y^{l,3}_1H^{l,3,1}_2 k(t^{l,3}_1+t^{l,3,1}_2)\\
% &+Y^{l,3}_2H^{l,3,1}_1 k(t^{l,3}_2+t^{l,3,1}_1)\\
% &+Y^{l,3}_1H^{l,3,1}_2 k(t^{l,3}_2+t^{l,3,1}_2)\\
% &+Y^{l,4}_1H^{l,4,1}_1 k(t^{l,4}_1+t^{l,4,1}_1)\\
% &+Y^{l,4}_1H^{l,4,1}_2 k(t^{l,4}_1+t^{l,4,1}_2)\\
% &+Y^{l,4}_2H^{l,4,1}_1 k(t^{l,4}_2+t^{l,4,1}_1)\\
% &+Y^{l,4}_1H^{l,4,1}_2 k(t^{l,4}_2+t^{l,4,1}_2)
% \end{align}

% which implies that for this case with two kernels per input, and two kernels per filter, the output $z_{l1}(t)$ is composed of $16$ kernels. In this case the index $i$ in \eqref{eq:Zi} runs from $1$ to $16$.

% This description of the last layer extends recursively across the previous layers of the network  towards the input $x(t)=y_{01}(t)$, 
% with the RELU operator applied at each layer transition

% \begin{align}\mathbf Y^{(l+1)n}(t)&=\text{RELU}(\mathbf Z^{ln})
% \end{align}


% Hence, the back propagation algorithm is formed by the following derivatives.

% \begin{align}
%     \nabla_Y \ell &= \mathbf K_{YY} \mathbf Y - \mathbf K_{YR} \mathbf R\\
%     \nabla_{\mathbf Z^{ln}} \mathbf Y^{(l+1) n} &= \mathbf 1\left[\mathbf {Z^{ln}}>0\right]\\
%     \nabla_{ H^{lmn}_p}  
%     Z^{ln}_i &= Y^{ln}_j     
% \end{align}

% \juan{Notice that, even if it is not as critical as with the Frechet derivatives, the number of knots also explodes. If the input has 2000 kernels, then here we have 16000 kernels in $z(t)$. And they will no be sit on the same knots in different layers and neurons. It is still better than with the Frechet derivatives, as at least here the filters keep having only $2$ kernels, but the chain rule is intractable. I think a pooling operator is imposed. }



% \juan{As opposed to the Frechet derivatives, the knots are assumed as given in these derivations. Alejandro R suggested a NN for the knots. Not clear which would be the input of this NN. In principle, it should be the input $x(t)$ of our KNN, but formally it does not live in a finite vector space, so it is not suitable for a standard NN. This is a pickle, because if we state that $x(t)$ can be converted into a finite space, then why using KNNs at all and not using a standard NN for everything.  }
% \juan{We are still trying to understand how the derivatives backpropagate when both the coefficients and knots are considered as variables. In principle we need to  consider the cross derivatives $\frac{d l^2}/{d td Y}$ and this could become seriously entangled.}








==> v35/sec_linear_operators.tex <==
%!TEX root =../compiler_paper.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   S E C T I O N   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{RKHS Convolutional Models with Integral Operators}\label{sec_rkhs_int_oper}

In the previous sections, we discussed RKHS convolutional signal models rooted in an algebra that encapsulates the geometric and algebraic properties of the functions in the RKHS -- Theorem~\ref{thm_general_A_rkhs} and~\ref{thm_asm_from_rkhs} --. \textcolor{green}{In this section, we build a generic ASM embedding the attributes of the RKHS entirely on the homomorphism of the ASM while using an ordinary polynomial algebra to define the filters. For this construction, we restrict our attention to those kernels whose properties can be linked to an integral operator.
}%green

\blue{KEEPING THIS HERE FOR MY WRITTING IN THIS SECTION
\begin{itemize}
%
%
\item The square integrability of $K(x,y)$ as a function in $L^{2}(\ccalX,\ccalY)$ with the Lebegue product measure guarantees that the integral operator $T_{K}$ is Hilbert-Schmidt~[Ref: A course in functional Analysis, Conway, page 267]. That is way we can work nicely with graphons despite the fact they are not strictly speaking a kernel. Another reference: [Bounded Integral operators on L2 spaces, Halmos, page 17]
%
%
\item Interestingly, in~[Bounded Integral operators on L2 spaces, Halmos] the box product is called \textit{convolution}
%
%
\item It is much more than a coincidence that we end up doing convolutions with kernels. When a Kernel can be written as $K(u,v)=\phi (u-v)$ where $\phi$ is measurable is called convolution kernel in~[Bounded Integral operators on L2 spaces, Halmos]. We always end up working with time delays. Measurability here requires belonging to $L_1$.
%
%
\item Whenever we work with a convolution kernel we can proof that the integral operator is \textbf{compact}~[Bounded Integral operators on L2 spaces, Halmos, page 73]
%
%
\item The Mercer condition is necessary to guarantee uniform convergence when expanding the kernel in terms of eigenvalues and eigenvectors. 
%
%
\item it seems we could get the same result considering Carleman kernels...(the semi-square-integrable kernels k, for which k(x, o)EL2(y) for almost every x)~[Bounded Integral operators on L2 spaces, Halmos, page 59]. WE NEED ONLY CARLEMAN KERNELS, IT DOES NOT HAVE TO BE MERCER. THIS MAKES SENSE AS THE GRAPHONS ALLOW FOR THE SAME NICE EXPANSION... I WILL UPDATE THIS LATER.... 
%
%
\end{itemize}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%  S U B  -   S E C T I O N   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS and Integral Operators}
\label{sub_sec_mk_int_op}


In some important families of RKHSs, the underlying kernel has properties linked to an integral operator, $T_{K}: L_{2}(\ccalX) \to L_{2}(\ccalX)$, given by
%
%
%
\begin{equation}\label{eq_sub_sec_rkhs_int_oper_1}
T_{K}\left\lbrace 
                         f
         \right\rbrace
        =
        \int_{\ccalX}
             K(u,v)f(v)d\mu(v),
\end{equation}
%
%
%
where $K: \ccalX\times\ccalX \to \mbC$ is a square integrable kernel of an RKHS $\ccalH\subset L_{2}(\ccalX)$. The symbol $\mu$ is a measure on $\ccalX$. If $K$ is square integrable in $\ccalX\times\ccalX$, i.e. $K\in L_{2}(\ccalX\times\ccalX)$, the operator $T_{K}$ in~\eqref{eq_sub_sec_rkhs_int_oper_1} is bounded, compact, and Hilbert-Schmidt~\cite[p.~267]{conway1994course}~\cite[p.~17,~59,~73]{halmos2012bounded}.


The RKHS linked to an integral operator as in~\eqref{eq_sub_sec_rkhs_int_oper_1} allows the systematic generation of other kernels using the so-called box product~\cite{paulsen2016introduction}. We recall that that for arbitrary functions $S_{1}, S_{2}\in L_{2}(\ccalX\times\ccalX)$ the box product, $\square$, between $S_{1}$ and $S_{2}$ is given by
%
%
%
\begin{equation}\label{eq_box_product}
 \left(
     S_{1}\square S_{2}
 \right)(u,v)
       =
       \int_{\ccalY}
             S_{1}(u,z)
             S_{2}(z,v)
                 d\mu (z)
                 .
\end{equation}
%
%
%




*************************\\
*************************\\


When considering two symbols, $S_{1}(u,v)$ and $S_{2}(u,v)$, one can use the \textit{box product} to produce another symbol with desirable properties~\cite{paulsen2016introduction}. If we denote by $\square$ the box product between $S_{1}(u,v)$ and $S_{2}(u,v)$, we have
%
%
%
\begin{equation}\label{eq_box_product}
 \left(
     S_{1}\square S_{2}
 \right)(u,v)
       =
       \int_{\ccalY}
             S_{1}(u,z)
             S_{2}(z,v)
                 d\mu (z)
                 .
\end{equation}
%
%
%
This operation is beneficial to build kernels -- in the sense of Definition~\ref{def_kernel} --. In fact,  if $S^{\ast}(u,v)=\overline{S(v,u)}$, then $S\square S^{\ast}$ is a kernel function~\cite[Theorem~11.2]{paulsen2016introduction}. Additionally, from~\cite{paulsen2016introduction} -- Proposition 2.13 -- we know that given a kernel $K(u,v)$, we can associate to it a unique RKHS, $\ccalH(K)$. 




************************\\
************************








\alejandropm{I AM HERE}




We will restrict ourselves to the case of continuous kernels, $K(u,v)$ introducing the following definition:

\begin{definition}[\cite{paulsen2016introduction}]
       \label{def_mercer_kernel}
       %
       Let $\ccalT$ be a compact subset of $\mbR^{N}$. A function $K: \ccalT\times\ccalT \to \mbC$ is called a Mercer kernel if it is a continuous, positive semidefinite function, i.e. a continuous kernel function.
       %
\end{definition}
The Mercer kernels will allow for a spectral eigen-decomposition, which together with the boundedness assumption on the operator $T_{K}$, will be necessary to prove that the standard polynomial algebra defined in \eqref{eq_polynomial_algebra} and \eqref{eq_polynomial_algebra_product} will induce valid filters operating over the signals in $\ccalH$, with $\ccalH$ as in Definition~\ref{def_kernel_succ}. %def_ASP
%the polynomial algebra will lead to valid elements of the $\ccalH$ in \ref{def_kernel_succ}.
% \begin{equation}\label{eq_box_product_mercer}
% \left(
%     K_{1}\square K_{2}
% \right)(u,v)
%       =
%       \int_{\ccalT}
%            K_{1}(u%,z)
%            K_{2}(z,v)
%                d\mu (z)
%                .
% \end{equation}
\subsection{Instantiation of the polynomial algebra in RKHSs}
The polynomial algebra $\ccalA_\ccalP$ in $\mbC$ is defined as follows:
% \begin{equation}\label{eq_polynomial_algebra}
%        \ccalA = \left\lbrace p_t = \sum_{r=0}^{R}a_{r}t^{r} \quad a_{r},t\in\mbC, \quad r,R\in\mbN \right\rbrace
% \end{equation}
\begin{align}
        \ccalA_\ccalP &= \left(\ccalP,\bullet,1\right) \label{eq_polynomial_namet}\\
       \ccalP &= \left\lbrace p_t = \sum_{r=0}^{R}a_{r}t^{r} \quad a_{r},t\in\mbC, \quad r,R\in\mbN \right\rbrace \label{eq_polynomial_algebra} \\
       \text{with product} &\left(\sum_{r=0}^{R}a_rt^r\right)\bullet\left(\sum_{s=0}^{S}b_st^s\right) = \sum_{l=0}^{R\text{+}S}\sum_{m=0}^{l}a_mb_{l\text{-}m}t^l \label{eq_polynomial_algebra_product}
\end{align}
which is associative and has an identity element $1$.

In order to map $\ccalA_\ccalP$ to a space of polynomials in $K$, we will extend the box product definitions to allow for powers of $K$:
% We will also extend the box product \eqref{eq:box_product_graphons}  definition to allow for a polynomial algebra, via the following definition:
%use the box product previously defined in \eqref{eq:box_product_graphons}, with $K$ being a Mercer kernel. We will also introduce the notation $r$-times box product of $K$ with itself as:
\begin{definition}
       \label{def_square_k_r}
       Given a Mercer kernel $K$ on $\ccalT\times\ccalT$, and $\square$ as in \eqref{eq:box_product_graphons}, we define the $r$-times box product of $K$ with itself as
       \begin{equation}\label{eq_A_square_r}
              K^{ r} = K \square K^{ r-1}
       \end{equation}
\end{definition}
% \begin{equation}\label{eq_A_square_r}
%        K^{ r} = K \square K^{ r-1}
% \end{equation}
% , this is the $r$-times box product of $K$ with itself.
Remembering the ASM structure described in Definition~\ref{def_ASP} and shown in Figure~\ref{fig_asp_model}, we can define the homomorphism $\rho$ from $\ccalA_\ccalP$ to the space $\ccalB(\ccalH)$ as follows:
\begin{definition}
       \label{def_rho_mercer}
       Given a Mercer kernel $K$ on $\ccalT\times\ccalT$, its associated RKHS $\ccalH$ in Definition~\ref{def_kernel_succ} and $\ccalA_\ccalP$ as in \eqref{eq_polynomial_algebra}; the homomorphism $\rho$ that takes the polynomial $p_t = \sum_{r=0}^{R}a_{r}t^{r}\in\ccalP$ to an operator in the set of signal operators $\ccalB(\ccalH)$ as in the ASM Definition~\ref{def_ASP} is:
       \begin{equation}\label{eq_rho_mercer}
              \rho(p_t) = p_K = \sum a_{r}K^{r+1}
       \end{equation}
\end{definition}

       % \begin{equation}\label{eq_rho_mercer}
%        \rho(p_t) = p_K(u,v) = \sum a_{r}K^{r+1}
% \end{equation}
This is, we represent the generic polynomials in $\ccalP$ by $p_t$, then, we obtain the expression for $p_K$ by replacing the powers of the independent variable in $p_t$ -- an ordinary polynomial -- with powers on $K$ as per \eqref{eq_A_square_r}. For instance, if $p_t= 1 + t + t^2$, then $p_K= K+ K^2 + K^{3}$. The need for the $r+1$ in the exponent instead of $r$ will be explained after defining the filter operation in the RKHS which we do next.

\begin{definition}\label{def_inner_product_kernel_instance}

If $p_t$ is a polynomial, $K$ is a Mercer kernel, with $\ccalH$ its RKHS as per Definition~\ref{def_kernel_succ}, and $x\in\ccalH$ is an input signal, then the filter output signal $y\in \ccalH$ of $p_K$ applied to the signal $x$ is defined as:
% \begin{equation} \label{eq_inner_product_kernel_instance}
%        y(v) = \rho(p_t) \{ x \} = \left\langle p_K(u,v), x(u) \right\rangle_{\ccalH}
% \end{equation}
\begin{align}
       y &= \rho(p_t) \{ x \}  \label{eq_inner_product_kernel_instance} \\
       \text{given by } y(v) &= \left\langle p_K(u,v), x(u) \right\rangle_{\ccalH} \label{eq_inner_product_kernel_instance_expanded}
\end{align}
Note that the inner product is applied over the variable $u$, so the output of the filter is a function of $v$.%for the inner product between $p_K(u,v)$, $u$ is the variable being integrated, so the output of the filter is a function of $v$.
\end{definition}

\begin{example}
       \textbf{Identity Filter}
       To validate $r+1$ as the appropiate exponent in \eqref{eq_rho_mercer}, consider the case where $p_t = 1$. In this case $p_K = K^1 = K$. Then from \eqref{eq_inner_product_kernel_instance_expanded} and \eqref{eq_inner_product_kernel} we have
       % Because $K$ is an RKHS \eqref{eq_linspan} and \eqref{eq_inner_product_kernel}, show that if we let $p_K = K$, then, using \eqref{eq_inner_product_kernel_instance},
\begin{equation}
       y(v) = \left\langle K(u,v), x(u) \right\rangle_{\ccalH} = x(v)
\end{equation}
This means that the filter instantiation $p_k=K$ is the identity operator in $\ccalH$, and the filter instantiation in \eqref{eq_rho_mercer} is consistent in the sense that $\rho(t^0) = \rho(1) = K^{0+1} = K$.
\end{example}
Now we are ready to state the following theorem, that shows that, for a fixed value of $v\in\ccalT$, $p_K(u,v)$ results in an element of the RKHS $\ccalH$. This makes \eqref{eq_inner_product_kernel_instance_expanded} in Definition \ref{def_inner_product_kernel_instance} a valid product that defines the filter.
% Now we are ready to state the following theorem, that shows that $p_k(u,v)$ when fixing $v$, results in an element of the RKHS and that makes Definition \ref{def_inner_product_kernel_instance} a valid product that defines the filters.
% which is the inner product of the kernel
%the inner product of the kernel
% This operations will allow us to build filters in the RKHS, using the polynomial algebra $\ccalA$. With this definitions we introduce the following theorem:

%Although $\ccalA_{\ccalH(K)}$ in~\eqref{eq_A_rkhs_gen} will have the central role in our analysis, the algebra we will introduce next will allow us to build signal processing models where one can link the attributes of the filtering with the decomposition of the signals in terms of the eigenvectors of the reproducing kernel.




%%--------------------------------------------
%%---------------- THEOREM -------------------
%%--------------------------------------------

\begin{theorem}
\label{thm_alg_RKHS_box_prod}
%
Let $K$ be a Mercer kernel on $\ccalT\times\ccalT$ such that its integral operator $T_K$ in \eqref{eq_sub_sec_rkhs_int_oper_tk} is bounded.%, and $\ccalA$ be the polynomial algebra in $\mbC$ defined by~\eqref{eq_polynomial_algebra}, with elements $p_t\in\ccalA$.

Let also $p_K=\rho(p_t)$ be the instantiation \eqref{eq_rho_mercer} of $p_t\in \ccalP$ with $\ccalA_\ccalP$ being the polynomial algebra in~\eqref{eq_polynomial_algebra}. For each $v\in\ccalT$ define $p_K^v$ such that $p_K^v(u) = p_K(u,v)$.%, be the filter instantiation of a filter $p_t\in\ccalA$, with $p_K(u,v)=\rho(p_t)$. Also, define $p_k^v$ from $p_k$ by fixing $v\in\ccalT$, i.e. $p_k^v(u) = p_k(u,v)$.

Then $p_K^v \in \ccalH$.
% \textbf{Corollary}
% The output of processing a signal using $p_K$ as a filter is given by~\eqref{eq_inner_product_kernel_instance}.
% Then $p_K$ is a kernel in the sense of Definition~\ref{def_kernel_succ}, $p_K(u,v) \text{ with }v \text{ fixed } \in \ccalH$, and the output of processing a signal using $p_K$ as a filter is given by~\eqref{eq_inner_product_kernel_instance}.
\end{theorem}

\begin{proof} See Appendix~\ref{proof_thm_alg_RKHS_box_prod} \end{proof}

\begin{corollary}
\label{corollary_alg_RKHS_box_prod}
%
With the hypothesis of Theorem~\ref{thm_alg_RKHS_box_prod}, $y=\langle p_K^v, x \rangle_{\ccalH}$ in Definition~\ref{def_inner_product_kernel_instance} is a valid filter output, i.e. it satisfies $y\in H$.
\end{corollary}

In addition to these two results, we show in Appendix \ref{proof_thm_alg_RKHS_box_prod}, that the space of filter instantiations $p_K$ form themselves an algebra with the identity operator defined in terms of the spectral decomposition of the Mercer kernel $K(u,v)$.
\subsection{Diffusive Kernels on Graphons}
%\leopoldo{WIP. Need more figures and examples.}
We will discuss the particular case of graphons, as introduced in \ref{sec:graphons_circ}. Note that if $W$ is continuous and bounded, then $K=W\square W^*$, as in \eqref{eq:graphon_kernel_WsqW} is a Mercer Kernel.

Moreover, since $\ccalT=[0,1]$ is compact, we have that the integral operator $T_K$ is bounded. This means that we can apply the filter in \eqref{eq_inner_product_kernel_instance_expanded} and the filter output $y(v) = \langle p_K(u,v), x(u) \rangle_{\ccalH}$ results to be a valid graphon signal.

% As introduced in section \ref{sec:graphons_circ}, and Proposition \ref{prop_WsqW}, given a graphon $W(u,v)$, we can define a kernel as $K(u,v)=W\square W^*$. We will again take $W(u,v) = \min(u,v)(1-\max(u,v))$ as an example. Note that as $W$ is continuous, $K$ is a Mercer kernel. The domain is $\ccalT = [0,1]$, which is compact which ensures the operator $T_K$ is bounded.

% This means that the inner product $y(v) = \langle p_K(u,v), x(u) \rangle_{\ccalH}$ is a valid filter output.

%placeholder figure
\begin{figure}[h]
       \centering
       \includegraphics[width=0.5\textwidth]{figures/placeholder.jpg}
       \caption{We will again take $W(u,v) = \min(u,v)(1-\max(u,v))$ as an example. Filtering a signal in $x\in\ccalH$ with $p_K = K + K^2 + K^3$, and $x=k(0.5,u)$, and therefore $\langle p_K(u,v), x(u) \rangle_{\ccalH} = \langle p_K^v(u), k(0.5,u) \rangle_{\ccalH} = p_K^v(0.5) = p_K(0.5,v)$. This filtering process results in a diffusion, as the input is propagated through a diffusing adjacency graph equivalent. This can be seen in the second half of the image.}
       \label{fig_graphon_filter}
\end{figure}

Figure \ref{fig_graphon_filter} shows the input and output of the filter $p_t = 1 + t + t^2$ instantiated as $p_K = K + K^2+K^3$ .
%Particularly, $x=k(0.5,u)$, and therefore
% $$\langle p_K(u,v), x(u) \rangle_{\ccalH} = \langle p_K^v(u), k(0.5,u) \rangle_{\ccalH} = p_K^v(0.5) = p_K(0.5,v)$$
Notice that, as $W$ is an extension of the graph adjacency matrix, and $\square$ an extension of matrix multiplication, $K= W\square W^*$ represents the graphon of \textit{two step neighbors}. Moreover, the filtering process given by \eqref{eq_inner_product_kernel_instance_expanded} results in a diffusion, because the input is propagated through a diffusing adjacency graph equivalent, and therefore $p_K$ is a diffusion filter.



% Once we have a Kernel, we can opt to build a filter using the polynomial algebra $\ccalA$, and filter with the Definition \ref{def_inner_product_kernel_instance} instead of the group operator defined in \ref{sec_conv_filt_rkhs}. This results in diffusion filters, in which higher exponents in the polynomial will result in more diffusion steps. This is illustrated in Figure \ref{fig_rkhs_on_graphon_ast}, where a signal in $\ccalH$ is filtered with $p_K = K+K^2$.
%%-------------- End of Theorem --------------
%\noindent We represent the generic polynomials in $\ccalA_{K}$ by $p\left(K \vert \square\right)$. Then, we obtain the expression for $p\left( K \vert \square\right)$ by replacing the powers of the independent variable in $p$ -- an ordinary polynomial -- with powers on $K$ considering the box product, $\square$. For instance, if $p(t)= 1 + t + t^2$, then $p(K\vert\square)= 1_{\ccalA_{K}}+ K + K^{\square 2}$.
%One of the interesting properties of $\ccalA_{K}$ is that certain subset are indeed elements of $\ccalH(K)$. This will allow us to develop convolutional models involving $\ccalA_{K}$ as the algebra and $\ccalH(K)$ as the vector space in an ASM. Due to the importance of this fact, we formalize it in the following result.
%%-----------------------------------------------------------
%%----------------  T H E O R E M  --------------------
%%-----------------------------------------------------------
% \begin{theorem}\label{thm_Ak_subsets_in_HK}
% %
% Let $p(t)$ be a polynomial and let $\ccalA_{K}$ be as defined in Theorem~\ref{thm_alg_RKHS_box_prod} for an RKHS $\ccalH(K)$. If
% %
% %
% $
% \boldsymbol{q}_{v}(K\vert\square)
% =
% \left(
% p
%     \left(
%              K\vert\square
%     \right)
%     \square
%     K
% \right)(u,v)
% $
% %
% %
% is the function -- on the variable $u$ -- obtained by fixing the value of  ``$v$" in the expression
% %
% %
% $
% \left(
% p
%     \left(
%              K\vert\square
%     \right)
%     \square
%     K
% \right)(u,v)
% \in\ccalA_{K}
% ,
% $
% %
% %
% then
% %
% %
% $
% \boldsymbol{q}_{v}(K\vert\square)
% \in
% \ccalH(K)
% $
% %
% %
% and
% %
% %
% $
% \left\langle
%                     \boldsymbol{q}_{v}(K\vert\square)
%                     ,
%                     \boldsymbol{x}
% \right\rangle_{\ccalH(K)}
% \in\ccalH(K)
% $
% %
% %
% with ``$v$" as the independent variable. Additionally, the map $\rho_{K}: \ccalA_{K} \to \ccalB(\ccalH(K))$ given by
% %
% %
% %
% \begin{equation}\label{eq_rho_Ak_Hk}
% \rho_{K}
%       \left(
%              p\left(
%                     K\vert\square
%                 \right)
%       \right)
%              \left\lbrace
%                    \boldsymbol{x}
%              \right\rbrace
%              =
%              \boldsymbol{y}(v)
%              =
%              \left\langle
%                      \boldsymbol{q}_{v}(K\vert\square)
%                     ,
%                     \boldsymbol{x}
%              \right\rangle_{\ccalH(K)}
%              ,
% \end{equation}
% %
% %
% %
% is a homomorphism.
% \end{theorem}
% \begin{proof} See Appendix~\ref{sub_sec_proof_thm_Ak_subsets_in_HK} \end{proof}
% %%------------  E N D   of Theorem   -----------------
% \red{
% \leopoldo{delete}
% From the results in Theorem~\ref{thm_Ak_subsets_in_HK}, we can obtain the convolutional model
% $(\ccalA_{K}, \ccalH(K), \rho_{K})$. While there could be multiple ways to build the homomorphism in an ASM involving $\ccalA_{K}$, the map in~\eqref{eq_rho_Ak_Hk} exhibits a natural connection with the ASM $(\mbC[t], L_{2}(\ccalT,\mu), \rho)$, where $\mbC[t]$ is the polynomial algebra and $\rho(t)=T_{K}$, with $T_{K}$ as in Theorem~\ref{thm_mercer}. Since this connection will be important for the discussion of RKHS convolutional models on graphons, we formalize it in the following theorem.
% %%-----------------------------------------------------------
% %%----------------  T H E O R E M  --------------------
% %%-----------------------------------------------------------
% \begin{theorem}\label{thm_alg_rkhs_vs_alg_classic}
% %
% Let $\ccalH(K)$ be an RKHS with Mercer reproducing kernel $K$. Let $T_{K}$ be as in Theorem~\ref{thm_mercer} and let $\ccalA_{K}$ be given according to Theorem~\ref{thm_alg_RKHS_box_prod}. Then, given the ASMs $(\ccalA_{K}, \ccalH(K), \rho_{K})$ and $(\mbC[t], L_{2}(\ccalT,\mu), \rho)$ with homorphisms $\rho_{K}$ given by~\eqref{eq_rho_Ak_Hk} and $\rho$ given by $\rho(t)=T_{K}$, we have that
% %
% %
% %
% \begin{equation}\label{eq_thm_alg_rkhs_vs_alg_classic}
% \rho\left(
%               p\left(
%                       t
%                 \right)
%        \right)
%              \left\lbrace
%                     \boldsymbol{x}
%              \right\rbrace
%              =
%                \rho_{K}
%                      \left(
%                            p\left(
%                                     K \vert \square
%                               \right)
%                      \right)
%                               \left\lbrace
%                                     \boldsymbol{x}
%                              \right\rbrace
%                              ,
% \end{equation}
% %
% %
% %
% for all $\boldsymbol{x}\in\ccalH(K)$ and any polynomial $p(t)\in\mbC[t]$.
% \end{theorem}
% \begin{proof} See Appendix~\ref{proof_thm_alg_rkhs_vs_alg_classic} \end{proof}
% %%-----------  E N D  of  Theorem  -------------------
% Theorem~\ref{thm_alg_rkhs_vs_alg_classic} establishes a direct connection between the common diffusions in an ASM and the filtering operation in an RKHS. It is possible to see that
% %
% %
% $
% \rho\left(
%               p\left(
%                       T_{K}
%                 \right)
%        \right)
%              \left\lbrace
%                     \boldsymbol{x}
%              \right\rbrace
%              \in
%              \ccalH(K)
% $
% %
% %
% for any $\boldsymbol{x}\in\ccalH(K)\subset L_{2}(\ccalT,\mu)$, with $\ccalH(K)$ being a subclass of signals in $L_{2}(\ccalT, \mu)$. This is, $\ccalH(K)$ remains invariant under the action of
% %
% %
% $
% \rho\left(
%               p\left(
%                       T_{K}
%                 \right)
%        \right)
%        .
% $
% %
% %
% This observation is key to quantify the effect of restricting the space of signals to be an RKHS. More specifically, we can say that if we require our space of signals to be an RKHS, we end up with a space that is invariant under the action of polynomial diffusions where $T_{K}$ is the shift operator.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{RKHS Algebras from Graphons}
% \label{sec_gphonsp_rkhs}
% %%-----------------------------------
% %%------------ FIGURE ---------------
% %%-----------------------------------

% \begin{figure*}
% %
% %--------- FIRST ROW ---------
% %
% \centering
%        \begin{subfigure}{.32\linewidth}
% 	   \centering
%           \includegraphics[width=0.8\textwidth]{./figures/graphon_rkhs/fig_6.pdf}
%        \end{subfigure}
%     	\begin{subfigure}{.32\linewidth}
% 		\centering
%             \includegraphics[width=1\textwidth]{./figures/graphon_rkhs/fig_5.pdf}
% \end{subfigure}
%     	\begin{subfigure}{.32\linewidth}
% 		\centering
%   \includegraphics[width=0.8\textwidth]{./figures/graphon_rkhs/fig_7.pdf}
% \end{subfigure}
% %
% %
% \caption{Depictions of the functions $\boldsymbol{k}_{v}(u)=K(u,v)$ in the RKHS graphon model considering the graphon $W(u,v)=\min(u,v)(1-\max(u,v))$. We show $K(u,v)$ with $u$ ranging from $0$ to $1$ and $v$ ranging from $0$ to $0.5$, $0.8$, and $0.4$. We restrict the values of $v$ to show how the behavior of $\boldsymbol{k}_{v}(u)$ concerning $K(u,v)=W\square W$. The kernel, $K(u,v)$, is determined using the box product between the graphon, $W$, with itself. We depict $\boldsymbol{k}_{0.5}(u)$ (left) and $\boldsymbol{k}_{0.8}(u)$ (left) and the result of their convolution, $\boldsymbol{k}_{0.5}(u)\bullet\boldsymbol{k}_{0.8}(u) = \boldsymbol{k}_{0.5\times 0.8}(u) =\boldsymbol{k}_{0.4}(u)$.}
% \label{fig_rkhs_on_graphon}
% \end{figure*}
% %%--------- End of Figure -----------
% Graphons have become a ubiquitous tool for processing information on graphs of large dimension~\cite{gphon_pooling_c,gphon_pooling_j,lovaz2012large}. A graphon is a symmetric bounded measurable function, $W: [0,1]^2 \to [0,1]$, that can be conceived as the limit of an adjacency matrix of a graph whose number of nodes and edges grows up to infinity~\cite{lovaz2012large}. For each graphon, $W(u,v)$, there is one associated integral operator $T_{W}:L^{2}([0,1])\to L^{2}([0,1])$ given by
% %
% %
% %
% \begin{equation}\label{eq_T_gphon_shift}
% T_{W}\left\lbrace
%                   \boldsymbol{x}
%               \right\rbrace
%       =
%       \int_{0}^{1}W(u,v)\boldsymbol{x}(u)du
%       .
% \end{equation}
% %
% %
% %
% The properties of $T_{W}$ can be used to study the properties of $W(u,v)$~\cite{lovaz2012large}. This is done by relating the spectral properties of $T$ with those of $W(u,v)$. More specifically, since $T_{W}$ is compact, normal, and Hilbert-Schmidt with eigenvalues $\lambda_i$ and eigenvectors $\boldsymbol{\varphi}_i$ -- which are orthonormal basis for $L_{2}([0,1])$ -- it can be shown that
% %
% %
% %
% \begin{equation}
% W(u,v) = \sum_{i=1}^{\infty}
%               \lambda_{i}
%               \boldsymbol{\varphi}_{i}(u)
%               \boldsymbol{\varphi}_{i}(v)
%               .
% \end{equation}
% %
% %
% %
% Additionally, one can leverage $T_{W}$ to define a convolutional signal processing model defined \textit{on} $W(u,v)$~\cite{gphon_pooling_c,gphon_pooling_j}. This can be done with the ASM $(\mbC[t],L_{2}([0,1]),\rho_{W})$, where $\mbC[t]$ is the polynomial algebra with independent variable $t$, $L_{2}([0,1])$ is the set of square integrable functions on $[0,1]$ with the Lebesgue measure, and $\rho_{W}: \mbC[t]\to\ccalB(L_{2}([0,1]))$ is the homomorphism that maps $t$ into $T_{W}$. Then, if $p(t)$ is a polynomial, the action of $\rho_{W}$ can be written as
% %
% %
% %
% \begin{equation}
% \rho_{W}\left( p(t) \right)
%        \left\lbrace
%               \boldsymbol{x}
%        \right\rbrace
%             =
%             p\left(
%                  T_{W}
%              \right)
%                     \left\lbrace
%                              \boldsymbol{x}
%                    \right\rbrace
%             .
% \end{equation}
% %
% %
% %
% Now we focus our attention on building an alternative convolutional model on graphons. To do so, we start recalling Theorem~\ref{thm_kernel_from_box_prod} considering as a symbol the graphon $W(u,v)$. Then, we have that given a graphon $W(u,v)$ we can obtain a kernel -- in the sense of Definition~\ref{def_kernel} -- utilizing the box product given by $K(u,v)= (W\square W)(u,v)$, which can be written in terms of the eigenvectors of $W(u,v)$ as we show in the following result.
% %%-----------------------------------
% %%----------- LEMMA -----------------
% %%-----------------------------------
% \begin{corollary}\label{corll_K_from_W}
% %
% Let $W(u,v)$ be a graphon with eigenvectors $\boldsymbol{\varphi}_{i}(u)$ and eigenvalues $\lambda_i$. Then, the function
% %
% %
% %
% \begin{equation}\label{eq_K_from_W}
% K(u,v) =
% W^{n\square}
% =
%         \sum_{i=1}^{\infty}
%              \lambda_{i}^{n}
%              \boldsymbol{\varphi}_{i}(u)
%              \boldsymbol{\varphi}_{i}(v)
%              ,
% \end{equation}
% %
% %
% %
% with $n\in\mbN$ and $n\geq 2$, is a kernel in the sense of Definition~\ref{def_kernel}. Additionally, if $K$ is continuous, $K$ is a Mercer kernel. $W^{n\square}$ indicates the $n$-times box product of $W$ with itself.
% \end{corollary}
% \begin{proof}
%     See Appendix~\ref{proof_corll_K_from_W}.
% \end{proof}
% %%-------- End of Lemma -------------
% With Corollary~\ref{corll_K_from_W} at hand we are ready to discuss convolutional graphon signal models relying on $\ccalA_{\ccalH(K)}$ and $\ccalA_{K}$. We start with an example where we show how the traditional graphon signal processing paradigm can be seen under the light of convolutional RKHS models.
% %%---------------------------------------------------------------
% %%------------------- E X A M P L E  -----------------------
% %%---------------------------------------------------------------
% \begin{example}\normalfont
% \label{ex_gphonsp_rkhs_AK}
% %
% Let $W$ be a graphon and let $K$ be the kernel given according to~\eqref{eq_K_from_W}. Let $\ccalH(K)$ be the RKHS with reproducing kernel $K$ given according to~\eqref{eq_HK_in_L2_as_rkhs} and let us recall that the classical convolutional signal model on graphons given by  $(\mbC[t],L_{2}([0,1]),\rho_{W})$ where $\rho_{W}$ is a homomorphism with $\rho_{W}(t)=T_{W}$. If we take into account that
% %
% %
% $
% T_{W}^{n}\lbrace \boldsymbol{x}\rbrace
% =
% T_{K}\lbrace \boldsymbol{x}\rbrace
% ,
% $
% %
% %
% we can see that for any polynomial $p(t)\in\mbC[t]$ we have
%  %
%  %
%  %
%  \begin{equation}\label{eq_ex_gphonsp_rkhs_AK_1}
% p\left(
%          T_{W}^{n}
%    \right)
%          \lbrace \boldsymbol{x}\rbrace
% =
% p\left(
%          T_{K}
%    \right)
%           \lbrace \boldsymbol{x}\rbrace
%           .
%  \end{equation}
% %
% %
% %
% Then, since $K$ is a Marcer Kernel, in the light of Theorem~\ref{thm_alg_rkhs_vs_alg_classic} we can see that
% %
% %
% %
% \begin{equation}\label{eq_ex_gphonsp_rkhs_AK_2}
% \rho_{W}\left(
%               p\left(
%                      t^{n}
%                 \right)
%        \right)
%              \left\lbrace
%                     \boldsymbol{x}
%              \right\rbrace
%              =
%               p\left(
%                    \rho_{W}\left( t \right)^{n}
%                 \right)
%              \left\lbrace
%                     \boldsymbol{x}
%              \right\rbrace
%              =
%                \rho_{K}
%                      \left(
%                            p\left(
%                                     K \vert \square
%                               \right)
%                      \right)
%                               \left\lbrace
%                                     \boldsymbol{x}
%                              \right\rbrace
%                       ,
% \end{equation}
% %
% %
% %
% for all $\boldsymbol{x}\in\ccalH(K)$.  This is, the RKHS convolutional model $(\ccalA_{K}, \ccalH(K), \rho_{K})$ is compatible with $(\mbC[t],L_{2}([0,1]),\rho_{W})$. Such compatibility, quantified by~\eqref{eq_ex_gphonsp_rkhs_AK_2}, emphasizes that the diffusions in $(\ccalA_{K}, \ccalH(K), \rho_{K})$ are $n$-times higher in order -- the order of the polynomial operator -- with respect to the diffusions in $(\ccalA_{K}, \ccalH(K), \rho_{K})$. This is, the same polynomial expression $p(t)$ leads to diffusions in $(\mbC[t],L_{2}([0,1]),\rho_{W})$ that are of higher order than those in $(\ccalA_{K}, \ccalH(K), \rho_{K})$. Notice that $\ccalH(K)$ is a proper subset of $L_{2}([0,1],\mu)$. This restriction of the class of signals considered comes as the price to pay for having an RKHS structure in $L_{2}([0,1],\mu)$.
% %
% \end{example}
% %%---------- E N D  of   E x a m p l e  -------------------
% One important aspect to remark about Corollary~\ref{corll_K_from_W} is the fact that different choices of $n$ in~\eqref{eq_K_from_W} lead to kernels that capture diffusions -- in the classical Gphon-SP model -- that have different selectivity. This can be observed from the fact that the function $\vert \lambda\vert^{n}$  concentrates around $\vert \lambda\vert =1$ when $[-1,1]$ which is where the spectrum of the graphon $W$ is contained -- see~\cite[p. 124, 131]{lovaz2012large}. This guarantees that the classical diffusions for large values of $n$ are more concentrated around the low frequencies, which by standard convention are associated to those eigenvalues close to $\vert \lambda\vert =1$. This shows that the algebra $\ccalA_{K}$ encapsulates naturally multiresolution attributes in its subsets of filters while allowing us to process signals in subsets of $\subset L_{2}([0,1],\mu)$ while exploiting the attributes of the RKHS $\ccalH(K)$.
% Now, we discuss an example of an RKHS convolutional model on graphs where we leverage the algebra $\ccalA_{\ccalH(K)}$.
% %%---------------------------------------------------------------
% %%------------------- E X A M P L E  -----------------------
% %%---------------------------------------------------------------
% \begin{example}\normalfont
% \label{ex_gphonsp_rkhs_AHK}
% %
% Considering $K$ as in~\eqref{eq_K_from_W} with $n=2$ we have an induced RKHS, $\ccalH (K)$, which defines a subset of functions in $L_{2}([0,1])$ and is given by~\eqref{eq_HK_in_L2_as_rkhs}. We can define a graphon convolutional signal model, $(\ccalA_{\ccalH(K)},\ccalH(K),\rho_{\ccalH(K)})$, where $\ccalA_{\ccalH(K)}$ is the algebra obtained from $\ccalH(K)$ according to Theorem~\ref{thm_general_A_rkhs} with $\theta (u,v) = uv
%     ,
%     ~\text{and}~
%     \delta = 1
%     .
% $
% %
% %
% with the homomorphism
% %
% %
% %
% \begin{equation}
% \rho_{\ccalH(K)}\left(
%                                 \sum_{u\in\ccalU}\alpha_{u}\boldsymbol{k}_{u}
%                           \right)
%     \left\lbrace
%                   \sum_{v\in\ccalV}\beta_{v}\boldsymbol{k}_{v}
%     \right\rbrace
%     =
%     \sum_{u\in\ccalU,v\in\ccalV}\alpha_{u}\beta_{v}\boldsymbol{k}_{uv}
%     .
% \end{equation}
% %
% %
% %
% In Fig.~\ref{fig_rkhs_on_graphon} we depict some of the functions $\boldsymbol{k}_{v}(u)$ in the RKHS graphon model. It is worth pointing out that we could have defined another convolutional model with $\ccalA_{\ccalH(K)}$ by considering $\theta(i,j)=(i+j)\text{mod}[0,1]$, i.e. the sum modulo 1 in the real numbers and choosing $0$ as the unit element of the sum.
% %
% \end{example}
% %%---------- E N D  of   E x a m p l e  -------------------
% Although Example~\ref{ex_gphonsp_rkhs_AHK} may seem counter intuitive when compared with the classical Gphon-SP model, it is still a type of convolutional model that can be used to perform scalable filtering and learning while keeping the advantages of working in an RKHS.
% \newpage
% \textcolor{white}{.}
% \newpage
%




==> v35/sec_preliminaries.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Background and Preliminaries}
\label{sec_background_and_prelim}

In this section, we discuss the preliminaries regarding RKHS and ASP. Before introducing the formal definition of an RKHS, let us state some basic notation. Let $\ccalX$ be a set, and let $\ccalF(\ccalX,\mbF)$ the set of functions from $\ccalX$ to the field $\mbF$. In our discussion we will have either $\mbF=\mbR$ or $\mbF=\mbC$. The set $\ccalF(\ccalX,\mbF)$ is a vector space with the ordinary sum of functions and multiplication of functions by scalars in $\mbF$. When considering any function in $\ccalF(\ccalX,\mbF)$ we use the notation $f(u)$ with $u\in\ccalX$. This will allow us to differentiate when discussing the structure of subspaces of $\ccalF(\ccalX,\mbF)$ and the role of the functions's domain, $\ccalX$. With this notation at hand we formally define RKHS following~\cite{paulsen2016introduction}.



%%-------------------------------------------------
%%------------ D E F I N I T I O N -----------
%%------------------------------------------------

\begin{definition}(\cite{paulsen2016introduction})\label{def_rkhs}
Let $\ccalX$ be a set. Then, $\ccalH\subset \ccalF(\ccalX,\mbF)$ is a reproducing kernel Hilbert space (RKHS) on $\ccalX$ if
%
%
\begin{enumerate}
    %
    %
    \item $\ccalH$ is a vector subspace of $\ccalF(\ccalX,\mbF)$
    %
    %
    \item $\ccalH$ is endowed with an inner product $\langle , \rangle_{\ccalH}$ with respect to which $\ccalH$ is a Hilbert space
    %
    %
    \item For every $u\in\ccalX$, the linear evaluation functional $E_{u}: \ccalH \to \mbF$, defined by $E_{u}(f)=f(u)$ is bounded.
    %
    %
\end{enumerate}

\end{definition}

%%------------ End of Definition -------------




If one takes into account the Riez representation theorem~\cite{paulsen2016introduction}, it is possible to show that for any $u\in\ccalX$ there exists a $k_{u}\in\ccalH$ such that $f(u)=\langle f, k_u \rangle_{\ccalH}$ for all $f\in\ccalH$. This also implies that $ E_{u}(f) = \langle f, k_u \rangle_{\ccalH}$. The function $k_u$ allows the definition of a \textit{Kernel} that encapsulates partly the properties of any RKHS. To show this, we introduce first the definition of a Kernel function. 



%%------------------------------------
%%--------- DEFINITION ---------------
%%------------------------------------

\begin{definition}[\cite{paulsen2016introduction}]
\label{def_kernel}
Let $\ccalX$ be a set and let $K: \ccalX \times \ccalX \to \mbC$ be a function of two variables. Then $K$ is called a kernel function provided that for every $n\in\mbN$ and for every choice of $n$ distinct points, $\{ u_1, \ldots, u_n \}\subset\ccalX$, the matrix $[K(u_i, u_j)]_{i,j}$ is positive semidefinite, which we denote by $[K(u_i, u_j)]_{i,j}\succcurlyeq 0$.
\end{definition}

%%-------- End of Definition ---------


As pointed out in~\cite{paulsen2016introduction}, given an RKHS, $\ccalH$, with evaluation functional $E_{v}(f)=\left\langle f, k_{v}(u)\right\rangle_{\ccalH}$, one can obtain a Kernel function, $K(u,v)$, by choosing $K(u,v)=k_{v}(u)$. Additionally, as we will show later $K(u,v)$ allows one to characterize fundamental attributes of the RKHS. We will refer to $K(u,v)=k_{v}(u)$ as the \textit{reproducing kernel} of $\ccalH$. Additionally, from now on, we denote an RKHS by $\ccalH(K)$, emphasizing the reproducing kernel associated with the RKHS. It is worth pointing out that  it is a common practice in the literature,  to start with a kernel function and then find an inner product that allows the definition of an RKHS~\cite{ghojogh2021reproducing,wainwright2019high}.


We now proceed to state a collection of results that will help us to characterize any RKHS. This will be of great value in subsequent sections where we study the algebraic properties linked to RKHS. 



%%---------------------------------------------
%%------------ THEOREM -----------------
%%---------------------------------------------

\begin{theorem}(\cite{paulsen2016introduction})\label{thm_density_ky}
Let $\ccalH$ be an RKHS with reproducing kernel $K(u,v)$. Then, the linear span of set of functions $k_{v}(x) = K(x,v)$ for $v\in\ccalX$ is dense in $\ccalH$.
\end{theorem}

%%-------- End of Theorem ----------------



Theorem~\ref{thm_density_ky} highlights the role of the $k_{v} (u)$ functions in an RKHS as an expansion set of functions for any element in $\ccalH$. In a pragmatic scenario,  Theorem~\ref{thm_density_ky} also implies that any element in $\ccalH$ can be approximated with an arbitrary degree of accuracy by a linear combination of functions $k_{v}$. Additionally, since $k_{v}$ is directly obtained from the kernel $K(u,v)$ associated with the RKHS there is a systematic way to generate the functions to approximate any element in $\ccalH$.  
 


Given an RKHS, $\ccalH(K)$, with kernel $K(u,v)$, one could expect the specific attributes of $K(u,v)$ to influence the functions in $\ccalH(K)$ given the fact that the set of functions $k_{v}(u) = K(u,v)$ is dense in $\ccalH(K)$. This is indeed the case for attributes such as continuity. It can be shown that if $K: \ccalX\times\ccalX\to\mbF$ is continuous -- considering the product topology -- then every function in $\ccalH(K)$ is continuous -- see Theorem 2.17 in~\cite{paulsen2016introduction} --, and where the notion of continuity in $\ccalH(K)$ is tied to the topology of $\ccalX$. Such association between the properties of $K$ and those of $\ccalH(K)$ is also strenghtened by the fact that any kernel $K:\ccalX\times\ccalX\to\mbF$ induces a unique RKHS -- Theorem 2.14 in~\cite{paulsen2016introduction} --.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  SUB - SECTION  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS and Integral Operators}
\label{sub_sec_rkhs_int_oper}

In this section, we discuss an important family of RKHS where the underlying kernel has properties characterized by an integral operator. In particular, we are interested in integral operators, $T_{S}$, given by
%
%
%
\begin{equation}\label{eq_sub_sec_rkhs_int_oper_1}
T_{S}\left\lbrace 
        f
 \right\rbrace
        =
        \int_{\ccalX}
             S(u,v)f(v)d\mu(v),
\end{equation}
%
%
%
where $S: \ccalX\times\ccalV \to \mbC$ is square integrable as a function of $v$, for any $u\in\ccalX$. The symbol $\mu$ is a measure on $\ccalV$. Then, for a given integral operator, $T_{S}$, we will refer to $S$ as the \textit{symbol} of $T_{S}$. When considering two symbols, $S_{1}(u,v)$ and $S_{2}(u,v)$, one can use the \textit{box product} to produce another symbol with desirable properties~\cite{paulsen2016introduction}. If we denote by $\square$ the box product between $S_{1}(u,v)$ and $S_{2}(u,v)$, we have
%
%
%
\begin{equation}\label{eq_box_product}
 \left(
     S_{1}\square S_{2}
 \right)(u,v)
       =
       \int_{\ccalY}
             S_{1}(u,z)
             S_{2}(z,v)
                 d\mu (z)
                 .
\end{equation}
%
%
%
This operation is beneficial to build kernels -- in the sense of Definition~\ref{def_kernel} --. In fact,  if $S^{\ast}(u,v)=\overline{S(v,u)}$, then $S\square S^{\ast}$ is a kernel function~\cite[Theorem~11.2]{paulsen2016introduction}. Additionally, from~\cite{paulsen2016introduction} -- Proposition 2.13 -- we know that given a kernel $K(u,v)$, we can associate to it a unique RKHS, $\ccalH(K)$. 



Among the kernels whose properties can be related to integral operators are \textit{Mercer kernels}, which are \textit{continuous} kernel functions. Given its importance we state formally their definition as follows.


%%---------------------------------------
%%------------ DEFINITION ---------------
%%---------------------------------------

\begin{definition}[\cite{paulsen2016introduction}]
\label{def_mercer_kernel}
%
Let $\ccalX$ be a compact subset of $\mbR^{N}$. A function $K: \ccalX\times\ccalX \to \mbC$ is called a Mercer kernel if it is a continuous, positive semidefinite function, i.e. a continuous kernel function. 
%
\end{definition}

%%--------- End of Definition -----------




For Mercer kernels, we can write $K$ as a decomposition in terms of the spectral decomposition of an associated integral operator. This point is emphasized in the following result. 



%%--------------------------------------
%%------------- THEOREM ----------------
%%--------------------------------------

\begin{theorem}[\cite{paulsen2016introduction}]
\label{thm_mercer}
%
Let $K$ be a Mercer kernel on $\ccalX$, let $\mu$ be a finite Borel measure with support $\ccalX$, and let $T_{K}: L_{2}(\ccalX,\mu)\to L_{2}(\ccalX,\mu)$ be the associated integral operator -- as in~\eqref{eq_sub_sec_rkhs_int_oper_1} --. Then there is a countable collection of orthonormal continuous functions $\{ \varphi_i \}_{i=1}^{\infty}$ on $\ccalX$ that are eigenvectors for $T_{K}$ with corresponding eigenvalues $\{ \sigma_i \}_{i=1}^{\infty}$ such that for every $g\in L_{2}(\ccalX,\mu)$ we have
%
%
%
\begin{equation}
T_{K}\{ g \}
      =
      \sum_{i=1}^{\infty}
             \sigma_{i}
                  \left\langle
                        g
                        ,
                        \varphi_i
                  \right\rangle_{L_{2}}
                  \varphi_{i}
                  .
\end{equation}
%
%
%
Furthermore,
%
%
%
\begin{equation}\label{eq_mercer_K_decomp}
K(u,v)
     =
      \sum_{i=1}^{\infty}
            \sigma_{i}
            \varphi_{i}(u)
            \varphi_{i}(v)
            .
\end{equation}
%
%
%
\end{theorem}

%%---------- End of Theorem ------------




Theorem~\ref{thm_mercer} provides us with the tools to characterize an RKHS in terms of an operator that can be leveraged to define convolutional signal models -- we will get to this point in Section~\ref{sec_conv_filt_rkhs}. Additionally, notice that the RKHS associated with the kernel in~\eqref{eq_mercer_K_decomp} is 
%
%
%
\begin{equation}\label{eq_HK_in_L2_as_rkhs}
\ccalH(K)
=
\left\lbrace 
       f\in L_{2}(\ccalX,\mu)
    \left\vert
        \sum_{i=1}^{\infty}
             \frac{
                   \langle
                      f
                      ,
                      \varphi_i
                   \rangle_{L_{2}}^{2}
                  }
                  {\sigma_i}
                  <
                  \infty
    \right.              
\right\rbrace
,
\end{equation}
%   
%
%
with inner product given by
%
%
%
\begin{equation}\label{eq_H_innerprod_vs_L2}
\left\langle
    f
    ,
    g
\right\rangle_{\ccalH(K)}
    =
    \sum_{i=1}^{\infty}
        \frac{
              \left\langle
                   f
                   ,
                   \varphi_i
              \right\rangle_{L_2}
              \left\langle
                   g
                   ,
                   \varphi_i
              \right\rangle_{L_2}
             }
        {\sigma_i}
        .
\end{equation}
%
%
%
We refer the reader to Appendix~\ref{sub_sec_Ts_Tk_relationship} for details on how these derivations are obtained. 



We know that when considering symbols and integral operators, we can build a kernel using the box product. If we also restrict to continuous symbols on compact domains, we obtain a Mercer kernel. While not obvious, one can expect to start with a Mercer kernel and then obtain a symbol that can be used to build a convolutional model. This observation is formalized in the following theorem from~\cite{paulsen2016introduction}.



%%---------------------------------------------------------------
%%------------------ T H E O R E M -----------------------
%%---------------------------------------------------------------

\begin{theorem}[Theorem 11.18 in~\cite{paulsen2016introduction}]
\label{thm_S_from_K_rkhs}
%
Let $K$ be a Mercer kernel on $\ccalX$, let $\mu$ be a finite Borel measure with support $\ccalX$ and let $\{ \varphi_i \}$ be the orthonormal family of eigenvectors corresponding to non zero eigenvalues $\{ \sigma_i \}$ of $T_{K}$ given by Theorem~\ref{thm_mercer}. Then:
%
%
\begin{enumerate}
  %
  \item $S(u,v)=\sum_{i}\sqrt{\sigma_i}\varphi_{i}(u)\varphi_{i}(v)$ is the symbol of a bounded integral operator, $T_{S}$, on $L_{2}(\ccalX,\mu)$;
  %  
  \item $T_{S}$ is a positive operator with $T_{S}^{2} = T_{K}$;
  %
  \item $\{ \sqrt{\lambda_i}\varphi_{i} \}$ is an orthonormal basis for $\ccalH(K)$;
  %
  \item $\ccalH(K)$ consists precisely of the functions $\sum_{i}\alpha_{i}\varphi_{i}(u)$ such that 
  %
  $
  \sum_{i}\left(\vert \alpha_{i}\vert^{2}/\lambda_{i}\right)<\infty.
  $
  %
\end{enumerate}
%
%
\end{theorem}

%%---------- End of Theorem -------------


Finally, we remark that, as we will show in subsequent sections, graphon signal processing is one of those scenarios where the symbol associated with the kernel in an RKHS, defines the attributes of a signal model, in particular the attributes of a graph-like domain whose number of nodes and edges is infinite. 



==> v35/sec_proof_of_theorems.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proofs and Extra Theorems}






















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%   S U B   -   S E C T I O N  %%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Auxiliary Results}
\label{sub_sec_aux_result}





















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm_alg_RKHS_box_prod}}
\label{proof_thm_alg_RKHS_box_prod}

\begin{proof}

We show that $\ccalA_{K}$ is an algebra. We start showing that $\ccalA_{K}$ is indeed a vector space. First, we check that the sum  in $\ccalA_{K}$ is closed. This follows  from
%
%
%
\begin{equation}
    \sum_{r=0}^{\infty}a_{r}K^{\square r}
+
    \sum_{r=0}^{\infty}b_{r}K^{\square r}
     =
     \sum_{r=0}^{\infty}
              \left( 
                     a_{r}+b_{r}
             \right)        
           K^{\square r}
           .
\end{equation}
%
%
%

Now, we show that the scalar multiplication is closed in $\ccalA_{K}$, which follows from
%
%
%
\begin{equation}
\alpha
       \sum_{r=0}^{\infty}a_{r}K^{\square r}
               =
                 \sum_{r=0}^{\infty}
                                 \left( 
                                        \alpha a_{r}
                                 \right)
                                          K^{\square r}   
                                          .   
\end{equation}
%
%
%

Now, we prove that ``$\bullet$" is an algebra product, which requires to check that
%
%
$
\left(
       \boldsymbol{x}
               \bullet
       \boldsymbol{y}
\right)
     \bullet\boldsymbol{z}
=
\boldsymbol{x}\bullet
\left(
        \boldsymbol{y}
                \bullet
        \boldsymbol{z}
\right)
,
$
%
%
for all $\boldsymbol{x}, \boldsymbol{y} , \boldsymbol{z}\in\ccalH$. Now, let us consider
%
%
%
\begin{equation}
\boldsymbol{x}
=
\left( 
    \sum_{r=0}^{\infty}x_{r}K^{\square r}
\right)
,
~
\boldsymbol{y}
=
\left( 
    \sum_{r=0}^{\infty}y_{r}K^{\square r}
\right)
,
\boldsymbol{z}
=
\left( 
     \sum_{r=0}^{\infty}z_{r}K^{\square r}
\right)
.
\end{equation}
%
%
%

Then, we start computing
%
%
%
\begin{equation}
\left(
\boldsymbol{x}\bullet\boldsymbol{y}
\right)
     \bullet\boldsymbol{z}
     =
\sum_{r,\ell,m=0}^{\infty}
         \left(
             x_{r}y_{\ell}
         \right)z_{m}
         \left( 
               K^{\square (r+\ell)}
         \right)
                 K^{\square m}
 .
\end{equation}
%
%
%
Since the scalar product and the sum are associative it then follows that
%
%
%
\begin{equation}
\left(
\boldsymbol{x}\bullet\boldsymbol{y}
\right)
     \bullet\boldsymbol{z}
     =
\sum_{r,\ell,m=0}^{\infty}
             x_{r}
         \left(    
             y_{\ell}
             z_{m}
         \right)
               K^{\square r}
         \left( 
               K^{\square (\ell+m)}
         \right)
=  
\boldsymbol{x}\bullet
\left(
      \boldsymbol{y}
       \bullet\boldsymbol{z}  
\right)           
 .
\end{equation}
%
%
%

Now, we show that $1_{\ccalA(K)}$ is indeed an identity element in $\ccalA_{K}$. We start taking into account
%
%
%
\begin{multline}
\boldsymbol{x}
     \bullet
1_{\ccalA_{K}}      
=
\left( 
    \sum_{r=0}^{\infty}x_{r}S^{\square r}
\right)
       \bullet
\left( 
    \sum_{i=0}^{\infty}\boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)
\right)  
\\    
=  
    \sum_{r=0}^{\infty}
              x_{r}
              \left( 
                    S^{\square r}  
                    \square
                    \sum_{i=0}^{\infty}\boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)
              \right)    
\end{multline}
%
%
%

By~\eqref{eq_thm_box_prod_spect_2} in Theorem~\ref{thm_box_prod_spect} we have
%
%
%
\begin{equation}
S^{\square r}
      =
        \sum_{i=0}^{\infty}
                          \lambda_{i}^{r}
                   \boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)
                   ,
\end{equation}
%
%
%
and by~\eqref{eq_thm_box_prod_spect_1} in Theorem~\ref{thm_box_prod_spect} we have
%
%
%
\begin{equation}\label{eq_proof_thm_alg_RKHS_box_prod_8}
                  \sum_{i=0}^{\infty}
                          \lambda_{i}^{r}
                          \boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)
                 \square            
                 \sum_{i=0}^{\infty}
                           \boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)    
               =       
                  \sum_{i=0}^{\infty}
                          \lambda_{i}^{r}
                          \boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)   
                          .
\end{equation}
%
%
%
Therefore, it follows that
%
%
%
\begin{equation}
\sum_{r=0}^{\infty}
              x_{r}
              \left( 
                    S^{\square r}  
                    \square
                    \sum_{i=0}^{\infty}\boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)
              \right)   
              =
              \sum_{r=0}^{\infty}
                       x_{r}
                       S^{\square r}
                       .
\end{equation}
%
%
%
Notice $\boldsymbol{x}\bullet 1_{\ccalA_{K}}=1_{\ccalA_{K}} \bullet \boldsymbol{x}$ follows  from the fact that the product in~\eqref{eq_proof_thm_alg_RKHS_box_prod_8} is commutative -- see~\eqref{eq_thm_box_prod_spect_1} in Theorem~\ref{thm_box_prod_spect}.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%   S U B  -  S E C T I O N    %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of Theorem~\ref{thm_Ak_subsets_in_HK}}
\label{sub_sec_proof_thm_Ak_subsets_in_HK}

We start taking into account that in the light of Theorem~\ref{thm_box_prod_spect} we have
%
%
%
\begin{equation}
\left(
p 
    \left(
             K\vert\square
    \right) 
    \square
    K
\right)(u,v)  
    =    
       \sum_{i=1}^{\infty}     
            p\left( 
                    \sigma_{i}
              \right)    
              \sigma_{i}      
              \boldsymbol{\varphi}_{i}(u)
              \boldsymbol{\varphi}_{i}(v)
              .
\end{equation}
%
%
%
Now, we evaluate the condition in~\eqref{eq_HK_in_L2_as_rkhs}  with
%
%
$
\boldsymbol{q}_{v}
           \left(
                  K\vert\square
            \right)             
$
%
%
to obtain
%
%
%    
\begin{multline}
\sum_{j=1}^{\infty}
            \frac{1}{\sigma_j}
             \left\langle
                             \sum_{i=1}^{\infty}     
                                           p\left( 
                                                   \sigma_{i}
                                             \right) 
                                             \sigma_{i}         
                                             \boldsymbol{\varphi}_{i}(u)
                                             \boldsymbol{\varphi}_{i}(v)
                     ,
                     \boldsymbol{\varphi}_{j}
             \right\rangle_{L_{2}}^{2}
             \\
             =
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                              \sigma_{i}
                           \boldsymbol{\varphi}_{j}(v)^{2}  
                           . 
\end{multline}     
%
%
%   
By using the H\"older inequality we have 
%
%
%
\begin{multline}
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                           \sigma_{i}   
                           \boldsymbol{\varphi}_{j}(v)^{2}                            
\leq 
                 \left( 
                        \max_{j}
                               p(\sigma_j)^{2}
                 \right)     
                 \left( 
                        \sum_{i=1}^{\infty}
                                  \sigma_{j}       
                                  \boldsymbol{\varphi}_{j}(v)^{2}  
                 \right)     
                 .         
\end{multline}
%
%
%
First, we notice that 
%
%
$
 \sum_{i=1}^{\infty}
                      \sigma_{j}       
                      \boldsymbol{\varphi}_{j}(v)^{2}  
=
K(v,v)  
,                    
$
%
%
and since $K$ is continuous, there exists $0<C<\infty$ such that $\vert K(u,v)\vert\leq C$ for all $u,v\in\ccalT$~\cite{paulsen2016introduction}. Second, notice that since $T_{K}$ is a bounded operator, the spectrum of $T_{K}$ is always bounded~\cite{conway1994course,aliprantis2002invitation}. Then, there exists $c>0$ such that $0\leq\sigma_{j}<c$. Therefore, if $p(t)$ is a polynomial we have that for any $t\in [0,c]$ there exists $D>0$ such that
%
%
$
p(t)^{2}<D
.
$
%
%
Putting this together we have that
%
%
$
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                           \sigma_{i}   
                           \boldsymbol{\varphi}_{j}(v)^{2}   
<
   \infty
   ,
$
%
%
which implies that $\boldsymbol{q}_{v}(K\vert\square)\in\ccalH(K)$.


Now, we use~\eqref{eq_HK_in_L2_as_rkhs} with the function 
%
%
$
 \left\langle 
                    p
                            \left(
                                   K\vert\square
                            \right)
                            \square
                            K
                    ,
                    \boldsymbol{x}
\right\rangle_{\ccalH(K)}
$
%
%
-- on the variable $v$ -- to obtain
%
%
%
\begin{multline}
\sum_{j=1}^{\infty}
            \frac{1}{\sigma_j}
             \left\langle
                             \sum_{i=1}^{\infty}     
                                           p\left( 
                                                   \sigma_{i}
                                             \right) 
                                             \sigma_{i}         
                                             \boldsymbol{\varphi}_{i}(v)
                                             \langle
                                                       \boldsymbol{\varphi}_{i}
                                                       ,
                                                       \boldsymbol{x}
                                             \rangle_{\ccalH(K)}
                     ,
                     \boldsymbol{\varphi}_{j}(v)
             \right\rangle_{L_{2}}^{2}
             \\
             =
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                              \sigma_{i}
                              \langle
                                        \boldsymbol{\varphi}_{i}
                                        ,
                                        \boldsymbol{x}
                             \rangle_{\ccalH(K)}^{2}
                           . 
\end{multline}  
%
%
%
Now, using the H\"older inequality we have
%
%
%
\begin{multline}
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                              \sigma_{i}
                              \langle
                                        \boldsymbol{\varphi}_{i}
                                        ,
                                        \boldsymbol{x}
                             \rangle_{\ccalH(K)}^{2}
                     \leq 
                     \\
                           \left( 
                                  \sum_{j=1}^{\infty}  
                                           \sigma_{i}
                                           \langle
                                                  \boldsymbol{\varphi}_{i}
                                                   ,
                                                  \boldsymbol{x}
                                           \rangle_{\ccalH(K)}^{2}
                           \right)    
                           \max_{j}
                           p(\sigma_{j})^{2}  
                           .
\end{multline}
%
%
%
Since $T_{K}$ is a bounded operator, the spectrum of $T_{K}$ is always boundedand there exists $c>0$ such that $0\leq\sigma_{j}<c$~\cite{conway1994course,aliprantis2002invitation}. Then, if $p(t)$ is a polynomial we have that for any $t\in [0,c]$ there exists $D>0$ such that $p(t)^{2}<D$. Additionally, taking into account that
%
%
%
\begin{equation}
\sum_{i=1}^{\infty}
        \sigma_{i}        
\left\langle 
       \boldsymbol{\varphi}_{i}
       ,
       \boldsymbol{x}
\right\rangle_{\ccalH(K)}^{2}
    =
\left\langle 
       \boldsymbol{x}
       ,
       \boldsymbol{x}
\right\rangle_{\ccalH(K)}^{2}    
=
\left\Vert 
     \boldsymbol{x}
\right\Vert_{\ccalH(K)}^{2}  
,   
\end{equation}
%
%
%
we have that
%
%
$
\sum_{j=1}^{\infty}  
                           p\left( 
                                    \sigma_{j}
                              \right)^{2} 
                              \sigma_{j}
                              \langle
                                        \boldsymbol{\varphi}_{j}
                                        ,
                                        \boldsymbol{x}
                             \rangle_{\ccalH(K)}^{2}
<
\infty
,
$
%
%
which implies that
%
%
$
 \left\langle 
                 p
                            \left(
                                   K\vert\square
                            \right)
                            \square
                            K
                    ,
                    \boldsymbol{x}
\right\rangle_{\ccalH(K)}
\in
\ccalH(K)
.
$
%
%

Now, we show that the map $\rho_{K}$ is a homomorphism. Notice that  $\rho_{K}$ is a linear map. We focus our attention on showing that $\rho_{K}$ preserves the product. We start taking into account that
%
%
%
\begin{multline}
\rho_{K}
     \left( 
            p(K\vert \square)
     \right)
             \left\lbrace 
                      \rho_{K}
                             \left( 
                                   q(K\vert \square)
                              \right)
                                      \left\lbrace 
                                             \boldsymbol{x}
                                      \right\rbrace
             \right\rbrace
=
\\
\left\langle
       \sum_{j=1}^{\infty}
                p(\sigma_{j})
                       \sigma_{j}
                       \boldsymbol{\varphi}_{j}(u)
                       \boldsymbol{\varphi}_{j}(v)
        ,
        \sum_{i=1}^{\infty}
                q(\sigma_{i})
                       \sigma_{i}
                       \boldsymbol{\varphi}_{i}(u)
                        \left\langle
                               \boldsymbol{\varphi}_{i}
                               ,
                               \boldsymbol{x}
                        \right\rangle_{\ccalH(K)}           
\right\rangle_{\ccalH(K)}    
.        
\end{multline}
%
%
%
Then, from the linearity properties of the inner product it follows that
%
%
%
\begin{multline}
\rho_{K}
     \left( 
            p(K\vert \square)
     \right)
             \left\lbrace 
                      \rho_{K}
                             \left( 
                                   q(K\vert \square)
                              \right)
                                      \left\lbrace 
                                             \boldsymbol{x}
                                      \right\rbrace
             \right\rbrace
=
\\
\sum_{j=1}^{\infty}
     p\left(
             \sigma_{j}
       \right)
     q\left(
             \sigma_{j}
       \right)  
     \sigma_{j}^{2}
     \boldsymbol{\varphi}_{j}(v)
             \left\langle
                     \boldsymbol{\varphi}_{j}
                     ,
                     \boldsymbol{x}
             \right\rangle_{\ccalH(K)}   
             \left\langle
                     \boldsymbol{\varphi}_{j}
                     ,
                     \boldsymbol{\varphi}_{j}
             \right\rangle_{\ccalH(K)}   
.        
\end{multline}
%
%
%
Now, taking into account that
%
%
$
\left\langle
      \boldsymbol{\varphi}_{j}
      ,
      \boldsymbol{\varphi}_{j}
\right\rangle_{\ccalH(K)}   
=
1/\sigma_{j}
$
%
%
-- see~\eqref{eq_norm_squared_in_HK_varphi},  Section~\ref{sub_sec_Ts_Tk_relationship} in the supplementary material -- it follows that
%
%
%
\begin{multline}
\rho_{K}
     \left( 
            p(K\vert \square)
     \right)
             \left\lbrace 
                      \rho_{K}
                             \left( 
                                   q(K\vert \square)
                              \right)
                                      \left\lbrace 
                                             \boldsymbol{x}
                                      \right\rbrace
             \right\rbrace
=
\\
\sum_{j=1}^{\infty}
     p\left(
             \sigma_{j}
       \right)
     q\left(
             \sigma_{j}
       \right)  
     \sigma_{j}
     \boldsymbol{\varphi}_{j}(v)
             \left\langle
                     \boldsymbol{\varphi}_{j}
                     ,
                     \boldsymbol{x}
             \right\rangle_{\ccalH(K)}    
.        
\end{multline}
%
%
%
Now, we take into account that
%
%
%
\begin{equation}
\rho_{K}
       \left( 
                  p(\square\vert K)
                      \square 
                  q(\square\vert K)
       \right)
               \left\lbrace 
                      \boldsymbol{x}
               \right\rbrace
               =
\left\langle 
     \left( 
         p(\square\vert K)
         \square 
         q(\square\vert K)
     \right)
     \square
     K
     ,
     \boldsymbol{x}
\right\rangle_{\ccalH(K)}
.
\end{equation}
%
%
%
From Theorem~\ref{thm_box_prod_spect} we know that
%
%
%
\begin{equation}
\left( 
     p(\square\vert K)
     \square 
     q(\square\vert K)
\right)
      \square
      K
=
\sum_{i=1}^{\infty}
      p(\sigma_{i})
      q(\sigma_{i})
      \sigma_{i}
      \boldsymbol{\varphi}_{i}(u)
      \boldsymbol{\varphi}_{i}(v)
      ,
\end{equation}
%
%
%
and therefore
%
%
%
\begin{equation}
	\rho_{K}
	\left( 
	p(\square\vert K)
	\square 
	q(\square\vert K)
	\right)
	\left\lbrace 
	\boldsymbol{x}
	\right\rbrace
	=
	\left\langle 
              \sum_{i=1}^{\infty}
                     p(\sigma_{i})
                     q(\sigma_{i})
                     \sigma_{i}
                     \boldsymbol{\varphi}_{i}(u)
                     \boldsymbol{\varphi}_{i}(v)
	,
	\boldsymbol{x}
	\right\rangle_{\ccalH(K)}
	.
\end{equation}
%
%
%
Developing the product this expression leads to
%
%
%
\begin{equation}
	\rho_{K}
	\left( 
	p(\square\vert K)
	\square 
	q(\square\vert K)
	\right)
	\left\lbrace 
	\boldsymbol{x}
	\right\rbrace
	=
	\sum_{i=1}^{\infty}
	p(\sigma_{i})
	q(\sigma_{i})
	\sigma_{i}
	\boldsymbol{\varphi}_{i}(v)
	\left\langle 
	\boldsymbol{\varphi}_{i}
	,
	\boldsymbol{x}
	\right\rangle_{\ccalH(K)}
	.
\end{equation}
%
%
%
Then, we have
%
%
%
\begin{equation}	
\rho_{K}
       \left( 
            p(K\vert \square)
       \right)
             \left\lbrace 
                   \rho_{K}
                          \left( 
                               q(K\vert \square)
                          \right)
                                \left\lbrace 
                                      \boldsymbol{x}
                                 \right\rbrace
             \right\rbrace  
= 
\rho_{K}
       \left( 
            p(\square\vert K)
            \square 
            q(\square\vert K)
       \right)
             \left\lbrace 
                    \boldsymbol{x}
             \right\rbrace  
             .          	
\end{equation}	 
%
%
%
\end{proof}





















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% S U B  -  S E C T I O N   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm_alg_rkhs_vs_alg_classic}}
\label{proof_thm_alg_rkhs_vs_alg_classic}
%
\begin{proof}
%	
By Theorem~\ref{thm_mercer} we know that
%
%
%
\begin{equation}\label{eq_proof_thm_alg_rkhs_vs_alg_classic_1}
p\left( 
       T_{K}
 \right)
       \left\lbrace 
             \boldsymbol{x}
       \right\rbrace	
=
\sum_{i=1}^{\infty}
          p\left(
                \sigma_{i}
           \right)       
           \boldsymbol{\varphi}_{i}(v)
           \left\langle 
                 \boldsymbol{\varphi}_{i}
                 ,
                 \boldsymbol{x}
           \right\rangle_{L_2} 
           .
\end{equation}
%
%
%
Since 
%
%
$
\langle 
     \boldsymbol{\varphi}_{i}
     ,
     \boldsymbol{x}
\rangle_{L_{2}}
=
\sigma_{i}   
\langle 
\boldsymbol{\varphi}_{i}
,
\boldsymbol{x}
\rangle_{\ccalH(K)}  
$
%
%
it follows that
%
%
%
\begin{equation}\label{eq_proof_thm_alg_rkhs_vs_alg_classic_2}
	p\left( 
	      T_{K}
	\right)
	    \left\lbrace 
	          \boldsymbol{x}
	    \right\rbrace	
=
	\sum_{i=1}^{\infty}
	        p\left(
	              \sigma_{i}
	         \right)       
	         \sigma_{i}
	         \boldsymbol{\varphi}_{i}(v)
	         \left\langle 
	              \boldsymbol{\varphi}_{i}
	              ,
	              \boldsymbol{x}
	         \right\rangle_{\ccalH(K)} 
	.
\end{equation}
%
%
%
Now, we recall from the definition of $\rho_{K}$ that
%
%
%
\begin{equation}\label{eq_proof_thm_alg_rkhs_vs_alg_classic_3}
\rho_{K}
	\left( 
	      p\left(
	           K\vert\square
	       \right)
	\right)
	      \left\lbrace 
	            \boldsymbol{x}
	      \right\rbrace
=
	\left\langle 
	      p(K\vert\square)\square K
	      ,
	      \boldsymbol{x}
	\right\rangle_{\ccalH(K)}
	,
\end{equation}
%
%
%
and from Theorem~\ref{thm_box_prod_spect} that
%
%
%
\begin{equation}\label{eq_proof_thm_alg_rkhs_vs_alg_classic_4}
p(K\vert\square)\square K
=
\sum_{i=1}^{\infty}
     p\left( 
           \sigma_{i}
      \right)
            \sigma_{i}
            \boldsymbol{\varphi}_{i}(u)
            \boldsymbol{\varphi}_{i}(v)	
            .
\end{equation}
%
%
%
Replacing~\eqref{eq_proof_thm_alg_rkhs_vs_alg_classic_4} into~\eqref{eq_proof_thm_alg_rkhs_vs_alg_classic_3}, distributing the product (inner), and comparing with~\eqref{eq_proof_thm_alg_rkhs_vs_alg_classic_2} it follows that
%
%
%
\begin{equation*}
p\left( 
      T_{K}
\right)
      \left\lbrace 
           \boldsymbol{x}
      \right\rbrace
      =
\rho_{K}
      \left( 
           p\left(
                K\vert\square
            \right)
      \right)
           \left\lbrace 
                 \boldsymbol{x}
           \right\rbrace      
           .
\end{equation*}
%
%
%
\end{proof}




























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%














































==> v35/sec_spectral_representations_algrkhs.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Spectral Representations}

\alejandropm{HERE I WILL RECHECK IF THIS DISCUSSION IS ACTUALLY NECESSARY}












